Virtuoso: Video-based Intelligence for real-time tuning on SOCs

Efficient and adaptive computer vision systems have been proposed to make computer vision tasks, such as image classification and object detection, optimized for embedded or mobile devices. These solutions, quite recent in their origin, focus on optimizing the model (a deep neural network, DNN) or the system by designing an adaptive system with approximation knobs. In spite of several recent efforts, we show that existing solutions suffer from two major drawbacks. First, the system does not consider energy consumption of the models while making a decision on which model to run. Second, the evaluation does not consider the practical scenario of contention on the device, due to other co-resident workloads. In this work, we propose an efficient and adaptive video object detection system, Virtuoso, which is jointly optimized for accuracy, energy efficiency, and latency. Underlying Virtuoso is a multi-branch execution kernel that is capable of running at different operating points in the accuracy-energy-latency axes, and a lightweight runtime scheduler to select the best fit execution branch to satisfy the user requirement. To fairly compare with Virtuoso, we benchmark 15 state-of-the-art or widely used protocols, including Faster R-CNN (FRCNN), YOLO v3, SSD, EfficientDet, SELSA, MEGA, REPP, FastAdapt, and our in-house adaptive variants of FRCNN+, YOLO+, SSD+, and EfficientDet+ (our variants have enhanced efficiency for mobiles). With this comprehensive benchmark, Virtuoso has shown superiority to all the above protocols, leading the accuracy frontier at every efficiency level on NVIDIA Jetson mobile GPUs. Specifically, Virtuoso has achieved an accuracy of 63.9%, which is more than 10% higher than some of the popular object detection models, FRCNN at 51.1%, and YOLO at 49.5%.

==> 5.5_temp_file_for_comments.tex <==
% Jay 10/26 Kept, but unused comments from section 5


% Memory is out of story.
%-------------------------------------------------------------------------------------
% Left for possible enhancement.
% Memory Profiling
% Jay : 10/17/2021 Seeing some contradictory results from double checking memory. Seems the memory foot print does not change while switching, and I currently don't know why. Might have to remove for now.
% As shown in Figure XX, SSD+ with imagesize 192 comes with the smallest memory footprint of 773.3MB, scaling up to 897.1MB with image size 320. For D0+, the peak memory consumption is 954MB, and D3+ the peak memory consumption is 3896MB. Observing the number of parameters in each model, SSD has 3.4M parameters, D0 has 3.9M parameters and D3 has 12M parameters. The trend in number of parameters roughly matches the peak memory consumption ratio between models, validating the peak memory consumption calculated using the native Tensorflow function.
% It should be noted that since the object tracker only runs on the CPU, tracker tuning knobs do not have any impact on the GPU memory footprint. Only detector imagesize knob for SSD+ and different models had impact on the memory footprint.
%-------------------------------------------------------------------------------------



% \begin{comment}
% \begin{table*}[ht!]
% \centering
% \small
% \begin{tabularx}{\textwidth}{|>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X
% |>{\hsize=.4\hsize\centering\arraybackslash}X|}
% \hline
% \textbf{Power Modes ID} & \textbf{FastAdapt} & \textbf{FRCNN+} & \textbf{YOLO+} & \textbf{FRCNN} & \textbf{YOLO} & \textbf{REPP w\ YOLOv3} & \textbf{MEGA} & \textbf{SELSA 50} & \textbf{SELSA 101}\\ 
% \hline
% \hline
% 0 & 2244 (J) & 2205 (J) & 2196 (J) & 6567 (J) & 14270 (J) & 3427 (J) & 5269 (J) & 12233 (J) & 14565 (J)\\
% \hline
% 2 & 2293 (J) & 2296 (J) & 2246 (J) & 6745 (J) & 14407 (J) & 3490 (J) & 5368 (J) & 12519 (J) & 14967 (J) \\
% \hline
% 4 & 2069 (J) & 2064 (J) & 1914 (J) & 5906 (J) & 11836 (J) & 3122 (J) & 4528 (J) & 10493 (J) & 12451 (J) \\
% \hline
% Average & 2202 (J) & 2189 (J) & 2119 (J) & 6406 (J) & 13504 (J) & 3346 (J) & 5055 (J) & 11748 (J) & 13995 (J) \\
% \hline
% \end{tabularx}\vspace{-0.5em}
% \caption{Energy consumption results for different video object detection solutions under different power modes on Jetson Xavier NX. We run all models on a randomly selected video dataset which includes 828 frames.}
% \label{tab:energy}
% \end{table*}

% \begin{table}[th!]
% \centering
% \small
% \scalebox{0.67}{
%     \begin{tabularx}{1.5\columnwidth}{|>{\hsize=.45\hsize\centering\arraybackslash}X
%     |>{\hsize=.45\hsize\centering\arraybackslash}X
%     |>{\hsize=.40\hsize\centering\arraybackslash}X
%     |>{\hsize=.40\hsize\centering\arraybackslash}X
%     |>{\hsize=.45\hsize\centering\arraybackslash}X
%     |>{\hsize=.45\hsize\centering\arraybackslash}X
%     |>{\hsize=.67\hsize\centering\arraybackslash}X
%     |>{\hsize=.57\hsize\centering\arraybackslash}X
%     |>{\hsize=.53\hsize\centering\arraybackslash}X
%     |>{\hsize=.45\hsize\centering\arraybackslash}X
%     |>{\hsize=.6\hsize\centering\arraybackslash}X
%     |>{\hsize=.45\hsize\centering\arraybackslash}X
%     |>{\hsize=.45\hsize\centering\arraybackslash}X
%     |>{\hsize=.45\hsize\centering\arraybackslash}X|}
%     \hline
%     \textbf{Power Modes} & \textit{Fast Adapt} & \textit{FRCNN+} & \textit{YOLO+} & \textit{SSD} & \textit{SSD+} & \textit{EffDet D0} & \textit{EffDet D3} & \textit{FRCNN} &\textit{YOLO} & \textit{REPP w\ YOLOv3} & \textit{MEGA} & \textit{SELSA 50} & \textit{SELSA 101}\\ 
%     \hline
%     \hline
%     0 & 2244 & 2205 & 2196 & 692 & 295 & 1050 & 4786 & 6567 & 14270 & 3427 & 5269 & 12233 & 14565\\
%     \hline
%     2 & 2293 & 2296 & 2246 & 757 & 346 & 1183 & 5050 & 6745 & 14407 & 3490 & 5368 & 12519 & 14967 \\
%     \hline
%     4 & 2069 & 2064 & 1914 & 716 & 347 & 1025 & 4323 & 5906 & 11836 & 3122 & 4528 & 10493 & 12451 \\
%     \hline
%     Avg & 2202 & 2189 & 2119& 722 & 329 & 1086 & 4720 & 6406 & 13504 & 3346 & 5055 & 11748 & 13995 \\
%     \hline
%     \end{tabularx}
% }
% \caption{Energy consumption (J) on Jetson Xavier NX.}
% \label{tab:energy}
% \end{table}
% \end{comment}


% Jay:  Left informative comments
% For our benchmark experiments, we implement the SOTA adaptive models for video object detection along with some popular models screened using the following criteria. 1) The code and model could be deployed on an NVIDIA Jetson TX2 board, which has the lowest computation power in our device selection. We used it at the peak power level of 15W, with an AI performance of 1.33 TFLOPS. 2) The model is open-sourced and the pretrained weights on the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) 2015 VID dataset~\cite{ILSVRC15} are available.


% Jay 10/18:Moved old comments / informative comments to below for readability.
% -------------------------------------------------------------------------------
% \begin{figure}[th!]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/energy.png}
%     \caption{Instantaneous power on Xavier NX.} 
%     % We initiate the NVIDIA tegrastats module followed by the video object detection models and report the power measured every 1 second during the inference.
%     % PW: Mentioned in text
%     \label{fig:energy}
% \end{figure}

% Jay : Kept informative comments
%The datasets include bounding box annotations of 30 object classes.
%, chosen by factors including movement type, level of video clutterness, and average number of object instance. 
%The datasets comes with a total of 5,354 videos, which comprises of 1,613,698 images. 
%The training dataset comes with 3,862 videos (1,122,397 frames) and the validation dataset is composed of 555 videos (176,126 frames). We report the accuracy of each model on the validation dataset.%which is by convention used as the test dataset, as labels of the test dataset are not released.

% This dataset was first released in the ImageNet Large Scale Visual Recognition Challenge 2015. The dataset includes bounding box annotations of 30 object classes, chosen by factors including movement type, level of video clutterness, and average number of object instance. The dataset comes with a total of 5,354 videos, which comprises of 1,613,698 images, on average there are 300 images per video. The dataset is divided into 3 parts: training set with 3,862 videos (1,122,397 images); validation set with 555 videos (176,126 images); and test set with 937 videos (315,175 images). The accuracy of each model is measured on the validation set of the dataset, which is by convention used as the test dataset, as labels of the test dataset are not released.
%To ensure fair comparison among different models, we choose the models that the original authors had provided corresponding to the pretrained weights on the ILSVRC 2015 VID dataset. 

%There are 30 classes in this dataset, which is a subset of the 200 basic-level categories of the full dataset for the image object detection competition. The classes in the ILSVRC 2015 VID dataset are carefully chosen by the organizer based on object scale, level of image clutterness, average number of object instances, etc. All classes are fully labeled for each clip.  




% Jay: Kept informative comments
%The energy consumption between timestamps $t=a$ and $t=b$ is computed as the summation of power within the interval (this is an approximation compared to the exact integration).


% \begin{equation}
%     % \small
%     \label{eq:energy-sum}
%     W\ (Joule) = \sum_{t = a}^{b} P(t)\ (Watt)
% \end{equation}

%As shown in Eq.~\ref{eq:energy}, the total energy consumption is the integral of power in the time dimension.
% \begin{equation}
%     % \small
%     \label{eq:energy}
%     W\ (Joule) = \int_{a}^{b} P(t)\ (Watt)\ dt
% \end{equation}
% %  \si(\watt)\ 
% \noindent where a is the start time and b is the end time. As we use a discrete time interval for {\em tegrastats}, Eq.~\ref{eq:energy} can be simplified to a sum form as shown in Eq.~\ref{eq:energy-sum}
% \begin{equation}
%     % \small
%     \label{eq:energy-sum}
%     W\ (Joule) = \sum_{t = a}^{b} P(t)\ (Watt)
% \end{equation}


% Jay : Keep informative comments.
% mAP measures both localization and classification accuracy by comparing output bounding boxes against ground-truth boxes using different Intersection-over-Union (IoU) thresholds. Formally, mAP is defined as the mean value of the APs for all classes, given by
% \begin{equation}
%     %\small
%     mAP = \frac{\sum_{n=1}^{N} AP_n}{N}
%     \label{eq:map}
% \end{equation}
% where $AP_n$ is the average precision of class $n$ with $N$ as the total number of classes

% \begin{equation}
%     \small
%     TP = True\ Positives\
%     (Predicted\ as\ positive\ as\ was\ correct)
%     \label{eq:tp}
% \end{equation}

% \begin{equation}
%     \small
%     FP = False\ Positives\ 
%     (Predicted\ as\ positive\ but\ was\ incorrect)
%     \label{fp}
% \end{equation}

% \begin{equation}
%     \small
%     FN = False\ Negatives\
%     (Failed\ to\ predict\ an\ object\ that\ was\ there)
%     \label{fn}
% \end{equation}

% \begin{equation}
%     \small
%     Precision = \frac{TP}{TP+FP}
%     \label{eq:precision}
% \end{equation}

% \begin{equation}
%     \small
%     Recall = \frac{TP}{TP+FN}
%     \label{eq:recall}
% \end{equation}

% \begin{equation}
%     \small
%     Intersection\ over\ Union\ (IoU) = \frac{Area\ of\ Overlap}{Area\ of\ Union}
%     \label{eq:iou}
% \end{equation}
% In object detection tasks, IoU is calculated by divide the area of overlap by area of union.
% Area of overlap is the intersection between the predicted bounding box and the ground-truth bounding box.
% Area of union is the area encompassed by both the predicted bounding box and the ground-truth bounding box.
% we calculate Precision and Recall using IoU value for a given IoU threshold. In this paper, we use 0.5 as the IoU threshold which means if the IoU value for a prediction is 0.7, then we classify the prediction as TP, if IoU is 0.3, we classify it as FP.

% \somali{define mAP mathematically}
% \saurabh{Explain what mAP is. Explain characteristics of the dataset, how many videos, length of each, etc.}
% \pengcheng{done}

==> 6-sec_conclusion_old_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is a deprecated version of the conclusion.
% Kept just in case.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Conclusion} \label{sec:conclusion}

\somali{The conclusion has a few too many numerical results and it becomes rambling. Keep the full version as a comment and then extract out maybe 3/4 of the more important results to highlight.}
\begin{comment}
\pengcheng{We have 4 dimensions to do comparison: object detection models, contention levels, devices, power modes. To compare each dimension, we need to fix other dimensions.}
\begin{enumerate}
    \item Different models, same board, same contention level, same max power mode
    % 100 \% power correct? \PW{04/05/2021 06:23 Yes}
    \item Different contention levels, same model, same device, same max power mode
    \item Different boards, same model, same contention level, same max power mode    
    \item 3 different power modes, same model, same device, no contention
\end{enumerate}
\end{comment}

In this paper, we benchmark state-of-the-art video object detection frameworks on leading edge mobile GPUs under different GPU contention and power-mode scenarios. We show the latency, accuracy, and power consumption of \name, our proposed multi-branch and adaptive video object detection framework, along with those of leading video object detection models under each scenario. 
% There are 3 main variables in our benchmarking platforms: devices, GPU contention levels, and power modes. 
% Thus, our work provides insight into the performance of these models under GPU resource-constrained or power-constrained scenarios. %The GPU contention generator is a program that can occupy a certain level of GPU resources which makes it is possible to simulate real applications. 
% For different power-modes, we use the API provided by NVIDIA for the Jetson class of devices. 
According to our observation, \name provides the best Pareto frontier of accuracy-vs-latency for all three of our boards and under all contention levels. However, if there are loose latency bounds, among adaptive models, FRCNN+ (\ie our implementation of FRCNN with a tracker) achieves the highest accuracy, while among non-adaptive models, SELSA outperforms all others. In addition, even compared with SSD+, which has an efficient backbone and tuning features, \name is able to outperform both accuracy and latency wise. For the most well-resourced board, the AGX Xavier, and under the most stringent latency requirement, \name is able to sustain 76 fps in the no-contention scenario, while on Xavier NX, it is 74 fps, and on Jetson TX2, it is 38 fps. 

Among the latest video object detection models, SELSA achieves the highest mAP (81.5\%, with ResNet-101) but also suffers from a high latency ($>$ 2 seconds per frame). Also, these models, SELSA, MEGA, and REPP, are not adaptive, and therefore, suffer in latency when faced with any level of contention. Models with an efficient backbone, SSD and EfficientDet-D0, are able to run with low latency (103 msec and 130 msec respectively on the TX2 board) on embedded devices with a reasonable accuracy, as they are aimed for efficiency. However, even with these efficient models, the impact of contention was significant showing up to $2\times$ the latency with no contention. In contrast, SSD+ which is our counterpart implementation of SSD with adaptive features, was able to handle contention without much increase in latency. We also perform energy consumption experiments and find that SSD, SSD+, and EfficientDet-D0 which has an efficient model design achieves superior performance in energy efficiency, while \name, FRCNN+, and YOLO+ follows up next and achieves significant performance compared to it's counterparts and other SOTA models. SELSA101, which showed the highest enery consumption, has more than 6X the energy consumption of these best-in-class protocols. Our further evaluation with different power modes shows that different power modes come with tradeoff between inference latency and energy consumption. Results suggest that if one uses the lowest power level on the boards, it does not always translate to equivalent energy savings, but still can save energy at the cost of inference latency.
\jay{Based on these benchmark results, we take one step further to utilize our findings and develop an adaptive video object detection system with a scheduler that considers the energy and memory dimension of the embedded devices. We were able to show dynamic switching of kernels with flexibility based on various user requirements, covering a wide spectrum of performance tradeoff from an inference time down to as low as 2.41 msec with D0+, and accuracy up to 63.87\% with D3+. Being more recently developed models, D0+ and D3+ were mostly superior to SSD+, while SSD+ had the advantage of low memory footprint and lower energy consumption.}
We hope that this work points to much further work in understanding the suitability of various object detection heads on embedded boards. The understanding must encompass varying levels of resource availability on these devices as well as varying power modes of operation available on these devices.

% Finally, we found that the different power modes of Xavier NX can be leveraged to limit the working frequency of CPU, GPU, and Memory modules, in turn saving energy. %SC04052021: which power modes and how much energy does it save by switching from the highest power mode to the lowest one that we tested on a sample board (Xavier NX?), everything else remaining the same.

==> old_files_temp/1-sec_introduction.tex <==
\section{Introduction}
\label{sec:intro}
Video analytic systems have seen widespread success in various domains, ranging from computationally heavy tasks such as recognizing faces for surveillance, to mobile applications such as detecting objects for mobile-based augmented reality (AR) to real-time systems, such as localizing pedestrians and cars for autonomous driving. A key component shared by these applications is the ability to detect objects in videos.

There is ongoing research on pushing the accuracy further for video object detection tasks. Some of the recent breakthroughs in video object detection involves frame aggregation, a technique that utilizes features from other frames during inference to enhance the detection results. SELSA~\cite{wu2019sequence} widens the window for selecting the frames for aggregation by not only selecting neighboring frames, but considering their semantic neighborhood. MEGA~\cite{chen2020memory} takes the work from SELSA one step further and adds global frame aggregation where frames from other videos, sharing semantic similarity, are also taken into account. While these techniques are performed during the runtime of the inference task, REPP~\cite{sabater2020robust} reuses the detection output from a baseline model to further post-process the detection output to enhance the detection results after the analysis of a video.
%\jay{04/06/2021 - 12:38 have added some other SOTA benchmarks as refs, shall I keep them?}
%SC04062021: No, keep it, this is very nicely done.
Other works make use of optical flow~\cite{zhu2017flow}, 
% which is a feature for motions present in the video object 
or techniques such as knowledge distillation~\cite{deng2019relation} that have not been commonly deployed in video object detection. These tasks are mostly geared toward accuracy and may need to leverage server-class machines or cloud-enterprises.
%\jay{04/06/2021 - 12:38 modified the connection with the below paragraph.}

On the other hand, mobile applications typically encounter limited energy or computational resources while still requiring strict latency guarantees. To improve the user's immersive experience (\eg in AR/VR games) or to give high-confidence outputs from streaming videos (\eg for pedestrian recognition in autonomous driving), such tasks must be performed in near real-time under stringent latency budgets of 33 msec or lower. 
%SC04052021: don't just say low, put the possible bounds
Even with advancements in mobile GPU devices, these devices lack the computation power that a server-class machine or a cloud enterprise provides. In response, following are some proposed innovations: applying reinforcement learning based neural architecture search (NAS) for a lightweight network (\eg ~\cite{tan2020efficientdet}), more efficient computation of the network~\cite{han2020ghostnet, howard2019searching} or using a dynamic pipeline adapting to content at runtime~\cite{fang2018nestdnn, xu2020approxdet}.

However, to our knowledge, no prior work has benchmarked state-of-the-art (SOTA) video object detection works, under varying resource contention on heterogeneous boards.
%
Further, no prior work has benchmarked these solutions on embedded devices for energy measurement, using different power budgets.
Thus, in this paper, we claim the following contributions:
We engineered \name --- a faster in-house variant of ApproxDet --- by optimizing the frame decoding and resizing modules and a better choice of library APIs using ApproxDet's opensource software release at \url{https://github.com/StarsThu2016/ApproxDet}. 
%SC04052021: sounds a tad vanilla without the details. It will look a lot better if you can spell out the specifics to show it was a significant engineering effort, which I anyway think it was
We also implemented FRCNN+ and YOLO+, which are engineered versions of FRCNN and YOLO, with image resizing as the adaptive approximation knob and with the addition of an object tracker (MedianFlow) for faster video object detection with lower jitter as in our framework \name\footnote{We experimentally determine that it is crucial to couple a tracking algorithm with the detection algorithm for the streaming analytics to keep up with the streaming video rate. In this setup, for a Group of Frames (GoF), object detection runs on one frame and the tracker on the remaining frames. A typical range for the size of GoF for \name is 1--100 frames, where 1 means detection only.}.
%Fast ApproxDet select from a list of candidates [1, 2, 4, 8, 20, 50, 100], where 1 means detection only.
We benchmark the SOTA models in video object detection on different mobile devices and benchmark under different GPU resource contention levels, or different power modes to investigate the impact of contention or power on video object detection solutions.
% We carried out energy consumption experiments on Xavier NX using 9 different models and 3 different power modes, provides insight into the real energy consumption performance of these video object detection works. Also validated the functionality of the power control APIs provided by NVIDIA.

% \pengcheng{04/05/2021 11:16 split the latency-accuracy experiments under contention on different devices and the energy consumption experiment under different power modes on one board}
% \pengcheng{merged}
%yin (04/05/2021): I don't think we need this level of details for contributions. Can we merge them into a single paragraph and highlight the systematic benchmark?

==> old_files_temp/2-sec_related_works.tex <==
\section{Related Work}
\label{sec:related-work}
% \jay{Here are some ideas for the related work section,
% \begin{enumerate}
%     \item Video Object Detection
%     \item Benchmark experiments or Contention?
% \end{enumerate}
% I have already tried to look for some examples with contention and object detection, but was hard to find.}
% \pengcheng{These papers are usually named as multiple tasks or multiple tenants DNN on a single device}

% We now provide some background on object detection and tracking on mobile devices and existing computer vision algorithms.
As a key problem in computer vision, video object detection seeks to locate object instances in video frames using bounding boxes and simultaneously classifying the instance into target categories with their class probabilities. The most widely used detection models adopt convolutional neural networks (CNNs), broken down into two parts: a backbone network that extracts features from images (\eg ResNet) and a detection network or head that classifies object regions based on the extracted features (\eg Faster R-CNN or YOLO). 
The detection network can be further categorized into two-stage~\cite{dai2016r, ren2015faster, tan2020efficientdet} or single-stage detectors~\cite{liu2016ssd, redmon2018yolov3, zhang2018single}. One representative work of two-stage detectors is Faster R-CNN (FRCNN)~\cite{ren2015faster}, which employs CNNs to extract image feature maps and feeds them into Region Proposal Networks (RPN) to generate regions-of-interest (RoIs) in the first stage. Then, in the second stage, the RoI pooling layer combines the feature maps from convolutional layers and the proposals from the RPN together to generate positive proposal feature maps and provide these to the classifier network. In contrast, single-stage detection solutions do not include the step of region proposal generation, rather directly classify a dense set of pre-defined regions. These models are efficiently optimized and often less accurate in challenging datasets. %For example, YOLO~\cite{redmon2016you} is a well-known one-stage network that simplifies the detection of objects as a regression problem by predicting bounding boxes and class probabilities directly without generating region proposals. 

A general trend in object detection has been to make deeper and more complex object detection networks in order to achieve higher accuracy such as in recent video object detection algorithms~\cite{wu2019sequence, chen2020memory, sabater2020robust}. However, these advancements in accuracy do not necessarily target making these algorithms more efficient in terms of the network size and the latency of the detection task. Further, in many real-world object detection tasks, the task has to be carried out in real-time on a computationally constrained platform such as a mobile or embedded device\footnote{We use the terms ``mobile device'' and ``embedded device" synonymously.}. In such cases, object detection, and more specifically in \name, video object detection becomes challenging because of the resource constraints and the often stringent latency budget (30--50 msec/frame) for acceptable video quality. 

\begin{comment}
%I commented this out for now because the writing is evolving and I want to send a version today before I head to bed [SC] :) You can make changes in this section after I ping you on the channel. 

% \pengcheng{04/06/2021 01:02 Added related benchmarking work, currently it is a draft version, I will keep searching and do more polish on this section}

\noindent{\bf Benchmarking of video object detection works on embedded devices}:
With the rise of video object detection coupled with the popularity of edge computing in recent years, video object detection tasks have been pushed to the edge/embedded devices where the data was collected. %Performing these works at the edge has lots of benefit, including but not limited to: lower cost in data transmission, lower end-to-end latency, more security for private data, etc. 
Edge computing was generally performed on embedded devices with limited computational power and thus user should have better a understanding on them by looking at a through benchmarking experiment. ~\cite{alyamkin2019low} has provided the the vision on low power computer vision works. However, none prior work has done that, ~\cite{clemons2011mevbench} has provided a benchmark suite with wide range of applications, however, none of SOTA works or latest device has been used, and its evaluation is not on GPU which is the most popular module for DNN based computer vision works. ~\cite{luo2018aiot} also provides a AI tasks benchmark suite based on Android and Raspberry-Pi, and covers different framworks like tensorflow and Caffe2. Nevertheless, there's no SOTA models in it and no evaluation was presented. ~\cite{ qasaimeh2021benchmarking} 
has conducted benchmarks of accuracy, latency, and energy of a wide range of vision kernels and neural networks on multiple embedded devices: ARM57 CPU, Nvidia Jetson TX2 and Xilinx ZCU102 FPGA. However, it only include 1 GPU enabled machine which is not comprehensive as embedded devices with GPU are very common nowadays. Also it hasn't included the SOTA models and it is not specific on video object detection as what we are focusing on in our work. Also, lots of video object detection solutions are designed by include multiple tuning knobs, ~\cite{ qasaimeh2021benchmarking} hasn't shown the accuracy-latency tradeoff on embedded devices. ~\cite{buckler2017reconfiguring} takes a more detailed look at the kernels of the image signal processing (ISP) pipeline, \eg it does a detailed investigation of how many stages of an ISP pipeline should be used, what algorithm the image sensor should use, and the quantization of the ADC. Consequently, it is less complete in terms of its coverage of the detection heads. It covers only one model for object detection, Faster R-CNN, which we also cover. They do not measure power, but use analytical formulae and simulations. ~\cite{zhu2018euphrates} optimizes the interaction between ISP and CNN in the CV pipeline is this. This also does the optimization in a SoC architecture specific manner. However, it is focused on video object detection.

% \saurabh{Give here why video object detection is important on mobiles, why it has been found to be challenging so far.}

% Yin (4/5/21): We should recognize those previous works on efficient object detection on mobiles (briefly mentioned in the intro). The main argument here is that despite these efforts, a systematic benchmark is missing for video object detection.

% \somali{DONE}
\end{comment}

==> old_files_temp/3-sec_technique.tex <==
\section{Benchmark Design}
\label{sec:tech}
% \pengcheng{Here we put:
% \begin{itemize}
%     \item Details of the models we selected
%     \item Hardware specifications for Jetson devices, and different power modes. [Done, see Table.~\ref{tab:jetson} and Table.~\ref{tab:nx-power-modes}]
%     \item Details of Contention Generator, we recalibrate it on NX and AGX. [Done, see Fig.~\ref{fig:recalibration}]
% \end{itemize}
% }

We now present the design of our benchmark. We introduce object detection methods considered in the benchmark, describe our evaluation metric, dataset, and embedded devices, and present our contention generator to create controlled levels of GPU contention.

\subsection{Selected Video Object Detection Models}
%introduce SOTA once in the beginning and reuse
%Yin (4/6/21): Can someone verify these numbers? I can't match them to the methods described here and those in the experiments.
We consider 6 SOTA adaptive models for video object detection with a total of 10 protocols (including variants of the same model) for our benchmark. These models are selected using the following criteria. 1) The code and model could be deployed on an Jetson TX2 board.
% , which has the lowest computation power in our device selection.
%\pengcheng{04/08/2021 11:59 commented for space}
% We used it at the peak power level of 15W, with an AI performance of 1.33 TFLOPS. 
2) The model is open-sourced and the pretrained weights on the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) 2015 VID dataset~\cite{ILSVRC15} are available. These models can be divided into two groups.


% For our benchmark experiments, we implement the SOTA adaptive models for video object detection along with some popular models screened using the following criteria. 1) The code and model could be deployed on an NVIDIA Jetson TX2 board, which has the lowest computation power in our device selection. We used it at the peak power level of 15W, with an AI performance of 1.33 TFLOPS. 2) The model is open-sourced and the pretrained weights on the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) 2015 VID dataset~\cite{ILSVRC15} are available.

% A total of 6 different models with a total of 10 protocols with variants are selected. These models can be divided into 2 groups:

%\jay{04/06/2021 - 12:48 changed this part without itemize and commented the original part below. Thought the content addition to the SOTA part will make it untidy.} %Looks good [SC]

\noindent{\bf Adaptive video object detection models}: We evaluate 3 adaptive video object detection models. %ApproxDet~\cite{xu2020approxdet} is our own faster implementation named \name. 
\name, which is our in-house variant of ApproxDet~\cite{xu2020approxdet}, sped up using our optimization in frame decoding and image resizing and improved library APIs to represent a state-of-the-art adaptive protocol.
FRCNN+ and YOLO+ in our improvement over FRCNN~\cite{ren2015faster} and YOLO~\cite{redmon2016you, redmon2018yolov3}.
%\pengcheng{04/08/2021 12:02 commented for space, we already have details in the following description}
%SC: good call
% on (1) using a medianflow tracker to track the objects (after the first frame in every group-of-frames) instead of running the slower object detection DNN for every frame and (2) a collection of model variants allowing different input shapes (both FRCNN+ and YOLO+) and number of region proposals (a feature in the region proposal-based framework, \ie FRCNN+, only).

%\jay{04/06/2021 - 1:02 Added more details on the selection and naming convention.}
%\squishlist
\noindent{\bf \name}: \name has five tuning knobs: 1) Image shape, 2) Number of region proposals, 3) Interval of the object detector being triggered (sampling interval), 4) Tracker type, and 5) Image downsampling ratio. %We carefully engineer our earlier ApproxDet implementation, making it 2-3 times faster, by optimizing the frame decoding and resizing modules and the library APIs.
%Instead of using opencv to resize the image, we use the list slicing in Python to resize the image for the object tracker (limited to ds=1, 2, 4, and other intergers).
%SC04052021: this may be a good place to summarize since we should have already fleshed this out earlier per my comment. Fill out XXX
% \PW 04/05/2021 17:45 Filled XXX, below is the info I got from Ran:
% ApproxDet on TX2: 80ms ~ 300ms latency requirement
% Fast ApproxDet on Tx2: 33.3ms ~ 100ms latency requirement
% Accuracy stay the same
\noindent{\bf FRCNN+}: We added two tuning knobs for FRCNN: 1) Image shape, and 2) Number of proposals. Medianflow  tracker~\cite{kalal2010forward} was employed for acceleration. With different combinations of the image shape and number of proposals, there are 28 branches with the shape in the following range [224, 320, 448, 576] and number of proposals in the following range [1, 3, 5, 10, 20, 50, 100]. We used the MedianFlow tracker to speed up while keeping a sampling interval of 8 frames for the object detector. 
% RX: no downsampling for the tracker, and a 4x downsampling ratio of the tracker for
%SC04052021: The above paragraph is not clear, I reworded: please check
% PC 04/05/2021 17:18 The sampling interval is for object detector to work at every 8th frames, during the interval (on the other 7 frames) we use object tracker. Rewrite.
\noindent{\bf YOLO+}: We included one tuning knob for YOLO, which is the shape of the input image, and also used it in tandem with the MedianFlow object tracker~\cite{kalal2010forward} for acceleration. There are a total of 12 branches with the shape in the following range [224, 256, 288, 320, 352, 384, 416, 448, 480, 512, 544, 576]. Similarly, object detection was triggered every 8 frames, which is the sampling interval knob in our \name implementation.
% , and the ratio of the tracker was set to 4
%\squishend

\noindent{\bf SOTA video object detection models}:
We also consider several latest video detection models. REPP comes with a total of three model (baseline) variants - YOLOv3, SELSA, FGFA - and only their implementation of the YOLOv3 baseline was able to run on a TX2 board. We address the baseline model as YOLOv3 to avoid confusion with our own YOLO implementations (PyTorch YOLO and YOLO+), and the full model with the post-processing technique as REPP+YOLOv3. MEGA is provided with two different backbone models with different levels of features usage. Here, we use the BASE model provided by the authors with ResNet-50 as the feature extractor, as this was the only configuration that could be run on the TX2 board. We call this model MEGA base. For SELSA, we utilize ResNet-50 and ResNet-101, with the corresponding variants referred to as SELSA 50 and SELSA 101.

% \begin{itemize}
%     \item Adaptive video object detection models: ApproxDet~\cite{xu2020approxdet} in our own faster implementation named \name, FRCNN-default~\cite{ren2015faster} with ResNet 50 as a backbone, YOLO-default~\cite{redmon2016you, redmon2018yolov3}, FRCNN+ and YOLO+ in our own improvement over FRCNN and YOLO on (1) using a medianflow tracker to track the objects (after the first frame in every group-of-frames) instead of running the slower object detection DNN for every frame and (2) a collection of model variants allowing different input shapes (both FRCNN+ and YOLO+) and number of region proposals (a feature in the region proposal-based framework, \ie FRCNN+, only).
%     \item SOTA video object detection models: 
%     YOLOv3 base provided by the authors of REPP~\cite{sabater2020robust}, REPP with YOLOv3, MEGA base~\cite{chen2020memory} with ResNet 50 as backbone, SELSA~\cite{wu2019sequence} with ResNet 50 as backbone, and SELSA with ResNet 101 as backbone.
% \end{itemize}
% \somali{can you say what the improvements specifically are -- I am guessing it is using the adaptive image size knob but spell it out for all three, \name, YOLO+, and FRCNN+}
% \jay{Will it be a good idea to mention that FRCNN and YOLO is also provided by the author with the pretrained weights?, Or shall we also add that we tune YOLO and FRCNN as well to have tuning knobs?}
% \saurabh{Which of the two is it or are both true?}
% \somali{explain how you adapt the two with the tuning knobs and what is the version provided by the authors from which you get the pre-trained weights.}
% \pengcheng{04/05/2021 04:13 Addressed most of the comments and left a PLACEHOLDER for Ran to check}
% \ran{Fixed.}


\begin{comment}
\begin{table*}[h!]
    \centering
    \small
    \begin{tabularx}{\textwidth}{|>{\hsize=.55\hsize\centering\arraybackslash}X
    |>{\hsize=1.15\hsize\centering\arraybackslash}X
    |>{\hsize=1.15\hsize\centering\arraybackslash}X
    |>{\hsize=1.15\hsize\centering\arraybackslash}X|}
    \hline
    \textbf{Models} & \textbf{Jetson TX2} & \textbf{Jetson Xavier NX} & \textbf{Jetson AGX Xavier}\\ 
    \hline
    \hline
    CPU & Dual-Core NVIDIA Denver 2 64-Bit CPU and Quad-Core ARM Cortex-A57 MPCore processor with max frequency at 2000MHz & 6-core NVIDIA Carmel ARMv8.2 64-bit CPU 6MB L2 + 4MB L3 with max frequency at 1900MHz & 8-core NVIDIA Carmel Armv8.2 64-bit CPU 8MB L2 + 4MB L3 with max frequency at 2265MHz \\
    \hline
    GPU & 256-core NVIDIA Pascal GPU with max frequency at 1300MHz & 384-core NVIDIA Volta GPU with 48 Tensor Cores with max frequency at 1100MHz & 512-core NVIDIA Volta GPU with 64 Tensor Cores with max frequency at 1377MHz \\
    \hline
    Memory & 8 GB 128-bit LPDDR4 59.7GB/s & 8 GB 128-bit LPDDR4x 51.2GB/s & 32 GB 256-bit LPDDR4x 136.5GB/s \\
    \hline
    Storage & 32 GB eMMC 5.1 & 16 GB eMMC 5.1 & 32 GB eMMC 5.1 \\
    \hline
    Power & 7.5W/15W & 10W/15W & 10W/15W/30W\\
    \hline
    DL Accelerator & - & 2x NVDLA Engines & 2x NVDLA Engines \\
    \hline
    AI Performance & 1.33 TFLOPS & 21 TOPS & 32 TOPS \\
    \hline
    Price & \$399 & \$399 & \$699 \\
    \hline
    \end{tabularx}
    \caption{Specifications for Jetson devices: TX2, Xavier NX, and AGX Xavier.}
    % ~\cite{tx2, xaviernx, agxxavier}
    \label{tab:jetson}
\end{table*}
\end{comment}

% We use CUDA 10 and cuDNN 7 as the base libraries for GPU-accelerated DNN primitives.
\subsection{Evaluation Metrics and Dataset}
\noindent {\bf Accuracy} of all models are measured with mean average precision (mAP), following the widely adapted evaluation protocol~\cite{lin2014microsoft} on the dataset. %mAP is defined as the mean of APs for all classes. AP is the area under the precision-recall curve that measures both localization and classification accuracy by comparing output bounding boxes against ground-truth boxes using different Intersection-over-Union (IoU) thresholds.


% mAP measures both localization and classification accuracy by comparing output bounding boxes against ground-truth boxes using different Intersection-over-Union (IoU) thresholds. Formally, mAP is defined as the mean value of the APs for all classes, given by
% \begin{equation}
%     %\small
%     mAP = \frac{\sum_{n=1}^{N} AP_n}{N}
%     \label{eq:map}
% \end{equation}
% where $AP_n$ is the average precision of class $n$ with $N$ as the total number of classes

% \begin{equation}
%     \small
%     TP = True\ Positives\
%     (Predicted\ as\ positive\ as\ was\ correct)
%     \label{eq:tp}
% \end{equation}

% \begin{equation}
%     \small
%     FP = False\ Positives\ 
%     (Predicted\ as\ positive\ but\ was\ incorrect)
%     \label{fp}
% \end{equation}

% \begin{equation}
%     \small
%     FN = False\ Negatives\
%     (Failed\ to\ predict\ an\ object\ that\ was\ there)
%     \label{fn}
% \end{equation}

% \begin{equation}
%     \small
%     Precision = \frac{TP}{TP+FP}
%     \label{eq:precision}
% \end{equation}

% \begin{equation}
%     \small
%     Recall = \frac{TP}{TP+FN}
%     \label{eq:recall}
% \end{equation}

% \begin{equation}
%     \small
%     Intersection\ over\ Union\ (IoU) = \frac{Area\ of\ Overlap}{Area\ of\ Union}
%     \label{eq:iou}
% \end{equation}
% In object detection tasks, IoU is calculated by divide the area of overlap by area of union.
% Area of overlap is the intersection between the predicted bounding box and the ground-truth bounding box.
% Area of union is the area encompassed by both the predicted bounding box and the ground-truth bounding box.
% we calculate Precision and Recall using IoU value for a given IoU threshold. In this paper, we use 0.5 as the IoU threshold which means if the IoU value for a prediction is 0.7, then we classify the prediction as TP, if IoU is 0.3, we classify it as FP.

% \somali{define mAP mathematically}
% \saurabh{Explain what mAP is. Explain characteristics of the dataset, how many videos, length of each, etc.}
% \pengcheng{done}

\noindent {\bf Latency} of all models are measured as per-frame latency during inference, further averaged to acquire the mean latency per frame. Each model can achieve a variety of accuracy-vs-latency points corresponding to different settings of the configuration parameters, specific to each protocol. Generally, for a usable range for each protocol, a setting that improves the accuracy leads to increased latency. This tradeoff space defines a set of Pareto optimal frontiers, as shown in Fig.~\ref{fig:pareto}, representing the accuracy and latency achieved by all the configuration knobs for a given protocol.
% \ref{fig:accuracy_latency_TX2},\ref{fig:accuracy_latency_NX},\ref{fig:accuracy_latency_AGX}.
%Here, the scatter points represent the accuracy and latency achieved by all the configuration knobs for a given protocol. A Pareto frontier defines the settings that are either superior in accuracy or latency against all other settings. In other words, for a given accuracy, a point on the Pareto frontier achieves the lowest latency. Alternately, for a given latency, a point on the Pareto frontier achieves the highest accuracy. Consequently, our evaluation only considers the settings of the models that are on the Pareto frontier. 

\begin{figure}
    \centering
    \includegraphics[width=0.50\columnwidth,clip]{figures/pareto-frontier.jpg}
    \caption{A Pareto frontier for the accuracy-latency tradeoff for a particular model, by varying its configuration knobs. The Pareto frontier has to be considered separately for each contention level.}
    \label{fig:pareto}
\end{figure}

% RX (4/8/2021): remove reference to save space ~\cite{tegrastats}
\noindent {\bf Energy consumption} is measured by using the API from NVIDIA - {\em tegrastats}. {\em Tegrastats} provides the information of current power usage for each module --- whether CPU or GPU. User can also specify the interval of the output from {\em tegrastats}. We use 1-sec interval in our experiments. This choice balances the need to collect accurate measurements at a fine time granularity while bounding the overhead of the measurement and corresponding impact on the performance of the main application. 
%The energy consumption between timestamps $t=a$ and $t=b$ is computed as the summation of power within the interval (this is an approximation compared to the exact integration).
\begin{comment}
\begin{equation}
    % \small
    \label{eq:energy-sum}
    W\ (Joule) = \sum_{t = a}^{b} P(t)\ (Watt)
\end{equation}
\end{comment}
%As shown in Eq.~\ref{eq:energy}, the total energy consumption is the integral of power in the time dimension.
% \begin{equation}
%     % \small
%     \label{eq:energy}
%     W\ (Joule) = \int_{a}^{b} P(t)\ (Watt)\ dt
% \end{equation}
% %  \si(\watt)\ 
% \noindent where a is the start time and b is the end time. As we use a discrete time interval for {\em tegrastats}, Eq.~\ref{eq:energy} can be simplified to a sum form as shown in Eq.~\ref{eq:energy-sum}
% \begin{equation}
%     % \small
%     \label{eq:energy-sum}
%     W\ (Joule) = \sum_{t = a}^{b} P(t)\ (Watt)
% \end{equation}

\noindent {\bf Dataset}: 
We use the ILSVRC 2015 VID validation dataset~\cite{ILSVRC15} as the benchmark dataset for the video object detection task to classify and localize the objects in 30 classes, and over 555 videos (176, 126 frames). 
%\pengcheng{04/08/2021 11:51 shorten for more space}
%The datasets include bounding box annotations of 30 object classes.
%, chosen by factors including movement type, level of video clutterness, and average number of object instance. 
%The datasets comes with a total of 5,354 videos, which comprises of 1,613,698 images. 
%The training dataset comes with 3,862 videos (1,122,397 frames) and the validation dataset is composed of 555 videos (176,126 frames). We report the accuracy of each model on the validation dataset.%which is by convention used as the test dataset, as labels of the test dataset are not released.

% This dataset was first released in the ImageNet Large Scale Visual Recognition Challenge 2015. The dataset includes bounding box annotations of 30 object classes, chosen by factors including movement type, level of video clutterness, and average number of object instance. The dataset comes with a total of 5,354 videos, which comprises of 1,613,698 images, on average there are 300 images per video. The dataset is divided into 3 parts: training set with 3,862 videos (1,122,397 images); validation set with 555 videos (176,126 images); and test set with 937 videos (315,175 images). The accuracy of each model is measured on the validation set of the dataset, which is by convention used as the test dataset, as labels of the test dataset are not released.
%To ensure fair comparison among different models, we choose the models that the original authors had provided corresponding to the pretrained weights on the ILSVRC 2015 VID dataset. 

%There are 30 classes in this dataset, which is a subset of the 200 basic-level categories of the full dataset for the image object detection competition. The classes in the ILSVRC 2015 VID dataset are carefully chosen by the organizer based on object scale, level of image clutterness, average number of object instances, etc. All classes are fully labeled for each clip.  


\subsection{Embedded Devices}
\label{subsec:embedded}
We selected several embedded devices in the Jetson class of mobile GPUs that represent the computationally most powerful embedded devices available for general release today. Each device has ``mobile GPUs'' in them. Specifically, three embedded devices are used to benchmark the video object detection models --- Jetson TX2, Jetson Xavier NX, and Jetson AGX Xavier
%\pengcheng{04/08/2021 11:42 changed for space}
% NVIDIA Jetson TX2, NVIDIA Jetson Xavier NX, and NVIDIA Jetson AGX Xavier
These devices have different levels of CPU, GPU, and Memory capacity, and thus provide a wide spectrum of resource constraints evaluated against our solution --- \name. The relation between their computational capacities is Jetson TX2 $<$ Jetson Xavier NX $<$ Jetson AGX Xavier. %Table~\ref{tab:jetson} gives the hardware specifications of these devices.
% RX (4/8/2021): remove unnecessary references to save space ~\cite{tx2}, ~\cite{xaviernx}, \cite{agxxavier}
% RX (4/8/2021): remove Table of specifications.

Each GPU and CPU on our chosen boards has a native Dynamic Voltage and Frequency Scaling (DVFS) functionality, which is enabled by default.
%SC040421: Put the link and cite it if there is a published source for confirming above. 
% RX (4/8/2021): remove unnecessary references to save space: ~\cite{jetson_guide}
DVFS provides a way to reduce (static and dynamic) power consumption of the embedded chips on the fly by scaling down the voltage and frequency based on the targeted performance requirements of the application. 
We disable DVFS by fixing the frequency of the modules at their max frequencies. We realized this through our detailed empirical investigations and found our step to be essential to generate reproducible results. 

\subsection{Contention Generator}

\begin{comment}
\begin{figure}[th!]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/nx-recalibration.png}
    \caption{Calibration of the GPU CG on Xavier NX.}
    \label{fig:nx-calibration}
    \includegraphics[width=0.7\columnwidth]{figures/agx-recalibration.png}
    \caption{Calibration of the GPU CG on AGX Xavier.}
    \label{fig:agx-calibration}
\end{figure}
\end{comment}

\begin{figure}[t]
    \centering
    \begin{minipage}[c]{0.48\columnwidth}
        \includegraphics[width=1\textwidth]{figures/nx-recalibration.png}
        \centerline{\small (a) Xavier NX}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.48\columnwidth}
        \includegraphics[width=1\textwidth]{figures/agx-recalibration.png}
        \centerline{\small (b) AGX Xavier}
    \end{minipage}
    \caption{Calibration of the GPU contention generator.} % on Xavier NX and AGX Xavier. 
    \label{fig:calibration}
\end{figure}
We benchmark object detection models for the contention experiments using a synthetic contention generator (CG) that we created.
% proposed in ApproxDet~\cite{xu2020approxdet}. 
%SC040421: Don't keep referencing the ApproxDet paper, otherwise the novelty factor of this paper is reduced. 
The CG simulates the processes that consumes GPU resources, which could co-exist with the object detection tasks. 
The CG occupies designated levels of resource on the GPU module by a percentage of the maximum capacity.
%\pengcheng{04/08/2021 11:42 commented for space}
% or on CPU by number of cores. 
%SC040421: Be specific and rewrite above - what does the contention generator do (matrix multiply with a configurable number of GPU threads?)? How do you control the level of contention?
% PW 04/05/2021 00:27 Added below
Each embedded device has a different GPU architecture and thus, different amounts of resources and computational ability. 
% The contention generator originally was only calibrated for the TX2 board, and we further re-calibrate the contention generator for the Xavier NX and the AGX Xavier board, to produce a consistent contention.
Our GPU CG performs
%\pengcheng{04/08/2021 11:42 commented for space}
add operation on a certain size of arrays by employing 
a CUDA kernel function. By changing the workload size of the CUDA program, we control the number of GPU cores that are kept busy in unit interval. For the observation of our calibration experiment, we use {\em tegrastats} to record the GPU utilization.
We calibrate the CG for each device so that 99\% GPU utilization at max frequency was achieved and all contention values less than that use a proportionately lesser percentage of workloads.
%SC040421: Verify. 
%SC04052021: so what I wrote above is verified, can you put verified so I know :) with initials/date
We show the offline profiling experiment results of the GPU CG on Xavier NX and AGX Xavier in Fig.~\ref{fig:calibration}.
% and ~\ref{fig:calibration}.
As can be seen, with the increasing CUDA program workload, the GPU utilization keeps increasing and finally saturates at 99\% when the workload is large enough.
%\pengcheng{04/08/2021 11:42 commented for space}
% One thing to mention here is that 99\% is the max GPU utilization that users can achieve on Jetson devices. 
% \pengcheng{04/08/2021 11:42 commented for space}
After the offline profiling experiment, we choose 12 discrete levels [0\%, 1\%, 10\%, 20\%, 30\%, 40\%, 50\%, 60\%, 70\%, 80\%, 90\%, 99\%] to serve as the CG's calibrated output, and accordingly, map to 12 internal parameters that correspond to the size of the workloads in the CG. 
%SC04052021: what are these internal parameters, can you put here in commented form for my curiosity
% PW 04/05/2021 17:39 Verified. We give the CG a target, for example 20%, that will map to a interval parameter for the CUDA program to run.



% \begin{figure}[h]
%     \centering  

% \end{figure}

% PW 04/05/2021 00:03 MoveD all the below content to corresponding evaluation section
% We find empirically that there is saturation when the contention generator is run at any level above 50\%. 
%SC040421: If you have space, add the plot where 50\% and 90\% contentions give the same values for latency and point here to that plot. 
% For all the experiments that have contention, the contention generator is first activated for 10 seconds to achieve a stable state, and then the object detection models are initiated (and measurements done).

%maybe total energy and gpu socket cost for each gpu contention level on each board.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Jay - moved commented/edited content to the bottom.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Contention}
% To simulate the real-world environment where applications may run on side-by-side, a contention generator is developed. The contention generator occupies designated levels of contention on the CPU or GPU by a percentage of the maximum capacity. Each board has different specifications for CPU and GPU, and for each board, calibration experiments are performed to ensure that the desired level of contention is observed.

% \subsection{Main Experiments - In Progress}
% \subsubsection{Implementation}
% % RX (3/29/2021): SSD-MobileNetv3, and v2-MnasFPN are commented.
% For all six baselines, we use the pretrained weights released by the original authors. ApproxDet+, Faster R-CNN, and YOLOv3 are trained on a 1\% subsampled ILSVRC 2015 VID training dataset, while SELSA, MEGA, and REPP are trained with a combination of ILSVRC 2015 VID and 2014 DET datasets.

% \subsubsection{Baselines}
% A Total of seven baseline models for object detection task is selected.
% \begin{enumerate}
%     \item ApproxDet+
%     \item Faster R-CNN~\cite{ren2016faster}
%     \item YOLOv3~\cite{redmon2016you}\footnote{For the implementationm, the PyTorch third party implementation is used.~\cite{yolo_source}} 
%     \item SELSA~\cite{wu2019sequence}
%     \item MEGA~\cite{chen2020memory}
%     \item REPP~\cite{sabater2020robust}
%     % RX (3/29/2021): These are models for images, and does not work on the VID dataset.
%     %\item SSD-MobileNetv3 \cite{liu2016ssd}
%     %\item SSD-MobileNetv2-MNasFPN - Might be included \cite{chen2020mnasfpn}
% \end{enumerate}

% \subsection{Prerequisites}
% This section covers simple outline on which experiments are performed before the main experiments, and what resources are being utilized.



==> old_files_temp/4-sec_evaluation.tex <==
\section{Implementation and Evaluation}
\label{sec:evaluation}

% PW  04/05/2021 01:352 Moved the below content to Sec3.1
% \subsection{Implementation}
% For \name, FRCNN, and YOLO, different approximation branches selected by the model based on available resources gives a Pareto-style result plot with varying accuracy and latency based on the selected approximation branch. 
% \jay{Will it be a good idea to mention that FRCNN and YOLO is also provided by the author with the pretrained weights?, Or shall we also add that we tune YOLO and FRCNN as well to have tuning knobs?}
% \saurabh{Which of the two is it or are both true?}
% \somali{explain how you adapt the two with the tuning knobs and what is the version provided by the authors from which you get the pre-trained weights.}
% \ran{FRCNN+ and YOLO+ are both collections of models. They are actually not adapting not all and we just report the Pareto frontier of each model variants.}

%\subsection{Experiment Setup}
%How we run each model on different devices:

% We evaluate each object detection model on our 3 embedded devices under [0, 20, 50, 90]\% GPU contention.
%     % (These experiments cover 3 dimensions: different models, different devices, different GPU contention levels.)
% We pick the Xavier NX board, which has the middle level of computational resources among our 3 devices, for the energy consumption experiment. We run all models on a randomly selected video dataset with 828 frames under 3 different power modes [0, 2, 4], as shown in Table~\ref{tab:nx-power-modes}. 
    % (This experiment covers 1 dimension with different power modes for one board)
    % \pengcheng{04/05/2021 01:40 Addressed}
    % \somali{what are the 3 power modes, as in the values}
% yin (04/05/2021): I'd suggest we merge this part into Section 3 (Benchmark Design).

% \pengcheng{04/05/2021 04:27 commented as we don't need to explain}
% \noindent\textbf{Metrics:} 
% Accuracy of each baseline model is calculated using a server machine 
% % - [spec - Auriga?] 
% % SB (4/4/21): No need for server specs
% as object detection outputs are deterministic and not impacted by hardware specifications or contention. 

\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g0.png}
        \centerline{\small (a) No contention}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g20.png}
        \centerline{\small (b) 20\% GPU contention (g20)}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g50.png}
        \centerline{\small (c) 50\% GPU contention (g50)}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g90.png}
        \centerline{\small (d) 90\% GPU contention (g90)}
    \end{minipage}
    \caption{Benchmarking the object detection algorithms on the NVIDIA Jetson TX2.}
    \label{fig:accuracy_latency_TX2}
\end{figure*}

\begin{comment}
\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g0_nx.png}
        \centerline{\small (a) No contention}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g20_nx.png}
        \centerline{\small (b) 20\% GPU contention}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g50_nx.png}
        \centerline{\small (c) 50\% GPU contention}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g90_nx.png}
        \centerline{\small (d) 90\% GPU contention}
    \end{minipage}
    \caption{[Jetson Xavier NX] Benchmarking the object detection algorithms on the NVIDIA Jetson Xavier NX.}
    \label{fig:accuracy_latency_NX}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g0_agx.png}
        \centerline{\small (a) No contention}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g20_agx.png}
        \centerline{\small (b) 20\% GPU contention}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g50_agx.png}
        \centerline{\small (c) 50\% GPU contention}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g90_agx.png}
        \centerline{\small (d) 90\% GPU contention}
    \end{minipage}
    \caption{[Jetson AGX Xavier] Benchmarking the object detection algorithms on the NVIDIA Jetson AGX Xavier.}
    \label{fig:accuracy_latency_AGX}
\end{figure*}
\end{comment}

\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g0_nx.png}
        \centerline{\small (a) Xavier NX, g0}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g50_nx.png}
        \centerline{\small (b) Xavier NX, g50}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g0_agx.png}
        \centerline{\small (c) AGX Xavier, g0}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.24\textwidth}
        \includegraphics[width=1\columnwidth]{figures/accuracy_p95_latency_g50_agx.png}
        \centerline{\small (d) AGX Xavier, g50}
    \end{minipage}
    \caption{Benchmarking the object detection algorithms on the NVIDIA Jetson Xavier NX and AGX Xavier.} %, under no contention (g0) and 50\% GPU contention (g50).}
    \label{fig:accuracy_latency_NXAGX}
\end{figure*}

% \todo[inline,color=olive]{saurabh: You can organize the experiments as: \\
% (1) Accuracy and latency experiments with classical models (FRCNN and YOLO) where we can change configuration knobs \\
% (2) Accuracy and latency experiments with SOTA {\em video detection} models (SELSA, MEGA, REPP) where we do not have any configuration knobs \\
% (3) Latency bar plots for various protocols \\
% (4) Energy plots (only for GPU) on NX and AGX
% }
% \pengcheng{04/05/2021 01:55 Reorganized}

% \pengcheng{04/05/2021 10:15 Canceled because they don't fit in one figure}
% \jay{Merge Ran's, Pengcheng's and Jay's plot under same device. Total of 3 plots with 3 devices.}
% \pengcheng{Good idea for saving space. Can Ran help on merging all the data into 3 figures?}
% \jay{Add the latency results from 1 or 2 more power modes - to be determined after the sync.}
\subsection{Accuracy and Latency Benchmark}

\noindent \textbf{Experiment setup}: We evaluate each object detection model on our 3 embedded devices under [0, 20, 50, 90]\% GPU contention on the ILSVRC VID 2015 validation set, as is standard practice. For adaptive video object detection models, we consider a streaming setting for inference with video frames fed one-by-one, and report the mean latency per video frame. For other methods, we use batch processing for inference. Fig.~\ref{fig:accuracy_latency_TX2}, ~\ref{fig:accuracy_latency_NXAGX}, and~\ref{fig:sota} summarize our main results. Power modes for our latency-accuracy experiments:
TX2: mode 0; Xavier NX: mode 2; AGX Xavier: mode 0.
\begin{comment}
the default modes are:
TX2: Power mode 3
Xavier NX: Power mode 3
AGX Xavier: Power mode 7
\end{comment}

% In Fig.~\ref{fig:accuracy_latency_TX2}, ~\ref{fig:accuracy_latency_NX}, ~\ref{fig:accuracy_latency_AGX}, and~\ref{fig:sota} we show the latency and accuracy experiment of adaptive video object detection models on ILSVRC VID 2015 validation dataset on different devices. We run these protocols in a streaming manner with video frames fed one-by-one, and report the mean latency per video frame.

\subsubsection{Adaptive Video Object Detection Models}
Fig.~\ref{fig:accuracy_latency_TX2} reports the accuracy and latency of all models with varying contention levels on the NVIDIA Jetson TX2 board.
%SC040421: Why did we switch from earlier 95\% latency metric (our earlier papers) to mean latency?
% RX: because mean latency of the best latency metric to benchmark a protocol (run-and-measure style) and however 95\% latency SLA is a metric for requirement, a scheduler should be attached to each protocol to select the right model (require-schedule-run-and-measure style). Since our paper is not motivated by guaranteeing the user experience of QoS but check the performance of models under contention and different devices, mean latency is a better choice.
In subfigure (a), we observe that \name has the lead in the accuracy-latency frontier over FRCNN+ and YOLO+ over a wide range of latency budgets, varying from 33.3 msec to 200 msec. For \name, the accuracy goes up to 49.8\% mAP, running at 142.7 msec per frame (roughly 7.0 fps) and the accuracy drops by 5.6\%, running at 37.9 fps. 
%SC040421: Are these accuracy numbers even roughly comparable to published numbers by the original authors. 
% RX: We are not able to compare becuase the original authors report accuracy on the COCO and VOC 2007 datasets. While our results are on the ILSVRC datasets.
For FRCNN+, it is able to achieve a similar accuracy to \name but the accuracy drops significantly (>15\%) as we dial up the speed to 20 fps. %This is because both the input shape and number of region proposals are crucial adaptive knobs to tune at runtime. 
On the other hand, YOLO+, though with lower accuracy given high latency budget (100 to 200 msec), wins at speed over FRCNN+ since the accuracy drop is 8\% from 150 msec speed to 50 msec speed. Finally, we also show that latency and accuracy of FRCNN and YOLO without our optimization in the figure, 
%SC04052021: default version is misleading, say which version. For example, the default version for YOLO is the darknet version, giving the relevant citations will suffice here.
% RX: I agree. We should use just use the term "YOLO" and remove the word "default" to indicate unchanged, as comparison to YOLO+ that is sped up by the tracker. 
where the latency axis is in log-scale. For FRCNN and YOLO, the latency is 693 and 1051 msec per frame while the accuracy is 51.1\% and 49.5\%, respectively.

In subfigures (b), (c), (d), we further measure the performance of these protocols under GPU contention. Compared to the subfigure (a), we observe that \name maintains the latency with reduced accuracy and superior to FRCNN+ and YOLO+, validating its claim of approximation (at runtime) to resource availability. Given a 50\% GPU contention, \name's accuracy drop is 7.8\% given a 30 fps speed and 1.0\% given a 5 fps speed. In contrast, FRCNN+ and YOLO+ are 1.5X-2X slower with 50\% to 90\% GPU contention.

% \pengcheng{04/05/2021 11:19 PLACEHOLDER: add more content to describe the results of latency-accuracy experiment on Xavier NX and AGX Xavier}
For the latency-accuracy experiments on Xavier NX and AGX Xavier, we set the latency budget as [20ms, 33ms, 50 ms, 100ms], in most cases \name is superior at both accuracy and latency than FRCNN+ and YOLO+.
% , thus it keep leading the performance. 
As we can see the results on Xavier NX from Fig.~\ref{fig:accuracy_latency_NXAGX}, in subfigure (a), \name achieves 49.3\% of accuracy with 59.3 msec per frame (16.9 fps), and accuracy drops to 43.9\% running at 35.2 fps. 
FRCNN+ is comparable to or even better than \name when the latency budget is sufficient. However, it drops quickly to 40.9\% when the latency budget decrease to 27.8 msec (36.0 fps). YOLO+ has a accuracy at 44.2\% when the latency budget is 52.2 msec (19.2 fps). We further add GPU contention for the latency-accuracy experiment, in subfigure (b), the overall latency of \name, FRCNN+, and YOLO+ increased as the contention increase from 0\% to 50\%. However, \name can still keep the fps about 10 fps when there is 50\%. 
%
Fig.~\ref{fig:accuracy_latency_NXAGX} (c) and (d) show that the models achieve roughly 2 times higher fps on AGX Xavier than on TX2. \name can achieve 47.5\% of accuracy at 49.8 fps. FRCNN+ can achieve 38.8\% accuracy at 57.3 fps and YOLO+ can achieve 40.0\% at 43.1 fps.
All 3 groups of experiments suggest that as contention increased, the accuracy is influenced and will drop accordingly.

% \pengcheng{04/06/2021 00:16 Addressed, please have a pass}
%SC04052021: this sentence above is vague, need numbers, how much better latency-wise and accuracy-wise or if there is a drop in accuracy by XXX\% but the mean latency drops only by XXX\%. Otherwise, this blurb does not add anything


\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.32\textwidth}
        \includegraphics[width=0.9\columnwidth]{figures/tx2_contention_performance.png}
        \centerline{\small (a) Jetson TX2}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.32\textwidth}
        \includegraphics[width=0.9\columnwidth]{figures/nx_contention_performance.png}
        \centerline{\small (b) Jetson Xavier NX}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.32\textwidth}
        \includegraphics[width=0.9\columnwidth]{figures/agx_contention_performance.png}
        \centerline{\small (c) Jetson AGX Xavier}
    \end{minipage}
    \caption{Benchmarking SOTA video object detection models on NVIDIA Jetson Devices under different contention levels. The accuracy measurements are the same among all boards and are as follows. YOLOv3: 51.25\% mAP, REPP+YOLOv3: 74.81\% mAP, MEGA base: 68.11\% mAP, SELSA 50: 77.31\% mAP, SELSA 101: 81.5\% mAP.}
    \label{fig:sota}
\end{figure*}

\subsubsection{SOTA Video Object Detection Models}
% We select a randomly selected video with sufficient number of frames (828 frames) to perform the latency experiments. For the first frame for each video, the latency measurement has a high overhead due to the model and input initialization having up to 10x times larger latency. Thus, we exclude the first frame from the evaluation.
% One exception is the REPP + YOLOv3 baseline, which involves post-processing on the whole detection output results. Only for the post-processing part in the REPP + YOLOv3 baseline, we measure the latency to run on the full video frames, and then divide the result by the number of frames to get the mean latency per frame.
% \pengcheng{04/05/2021 04:32 PLACEHOLDER: Use more numbers to describe the results of latency-accuracy experiment for SOTA baselines}
% \pengcheng{Addressed}
SOTA models (YOLOv3, REPP+YOLOv3, MEGA base, SELSA 50 and 101) focus on the accuracy of video object detection. As we can see from the caption of Fig.~\ref{fig:sota}, without latency budgets, they achieve higher mAP than adaptive models, ranging from 51.25\% to 81.5\%. However, they suffer from poor latency, further exacerbated under contention, showing up to 2X increased latency with contention over 50\%. This is because of their model sizes and inability to adapt to contention. 
% But this the trade-off that user need to do, either higher accuracy or lower latency. 
Among all models: YOLOv3 has the lowest latency along with a lowest mAP on all boards in line with prior works. SELSA 101 achieves the highest mAP but with the highest latency on all boards. In contrast, REPP+YOLOv3 has a superior mAP at 74.81\% while still maintaining a low latency. %The last point is that on all devices, these SOTA models follow a similar trend of increased accuracy with higher latency.

% \jay{Should the reason of 50\%, 90\% contention having similar results be explained?}
% \somali{no need to explain again because I have asked PengCheng to put the 50 versus 90 result in the technique section with the corresponding figure.}
% \pengcheng{Decided not to upload those figure as we run out of space}

% \pengcheng{04/05/2021 04:15 moved to conclusion section, should be more concise.}
% \ran{The following is the general speed comparison between TX2, AGX and NX. It is not related. }
% \textbf{Overall latency comparison between the 3 embedded devices in use for our experiments}:
% The overall results show that the trend in the latency plot per board is similar, and by further investigation, we observe that different boards roughly follow a latency difference, which can be expressed as a ratio. For example, here are the latency ratios for the 3 embedded devices we used for \name: the AGX board is 1.78 times faster than the NX board and 2.95 times faster than the TX2 board, and the NX board is 1.66 times faster than the TX2 board. The specifications provided for each board show the AI performance, and the ratio between AGX board and NX board roughly matches the TOPS (Tensor Operations per Second) ratio for the AGX and NX boards.
%\pengcheng{Moved this part from the tech section. The latency-accuracy for FastAdapt, FRCNN-Pareto, YOLO-Pareto, FRCNN-default, YOLO-default is done on 10\% of the test dataset}

%SC040821: Chopped for space
\begin{comment}
\begin{table}[ht!]
\centering
\small
\begin{tabularx}{\columnwidth}{|>{\hsize=0.4\hsize\centering\arraybackslash}X
|>{\hsize=.1\hsize\centering\arraybackslash}X
|>{\hsize=.1\hsize\centering\arraybackslash}X
|>{\hsize=.1\hsize\centering\arraybackslash}X
|>{\hsize=.1\hsize\centering\arraybackslash}X
|>{\hsize=.1\hsize\centering\arraybackslash}X|}
    \hline
    \textbf{Key Parameters} & \textbf{Power Mode 0} & \textbf{Power Mode 1} & \textbf{Power Mode 2} & \textbf{Power Mode 3} & \textbf{Power Mode 4}\\ 
    \hline
    \hline
    Power Budget & 15W & 15W & 15W & 10W & 10W \\
    \hline
    Online CPU Cores & 2 & 4 & 6 & 2 & 4 \\
    \hline
    Maximal CPU Frequency (MHz) & 1900 & 1400 & 1400 & 1500 & 1200 \\
    \hline
    Maximal GPU Frequency (MHz) & 1100 & 1100 & 1100 & 800 & 800 \\
    \hline
    %DL Accelerator cores & 2 & 2 & 2 & 2 & 2 \\
    %\hline
    Maximal DL Accelerator Frequency (MHz) & 1100 & 1100 & 1100 & 900 & 900 \\
    \hline
    %Maximal Memory Frequency (MHz) & 1600 & 1600 & 1600 & 1600 & 1600 \\
    %\hline
\end{tabularx}
\caption{Different Power Modes for Jetson Xavier NX.}
\label{tab:nx-power-modes}
\end{table}
\end{comment}
% RX (4/8/2021): remove reference to save space ~\cite{jetson_guide}

\begin{comment}
% RX (4/11/2021): no longer use this cross-column table, see the single-column version below.
\begin{table*}[ht!]
\centering
\small
\begin{tabularx}{\textwidth}{|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X|}
\hline
\textbf{Power Modes ID} & \textbf{FastAdapt} & \textbf{FRCNN+} & \textbf{YOLO+} & \textbf{FRCNN} & \textbf{YOLO} & \textbf{REPP w\ YOLOv3} & \textbf{MEGA} & \textbf{SELSA 50} & \textbf{SELSA 101}\\ 
\hline
\hline
0 & 2244 (J) & 2205 (J) & 2196 (J) & 6567 (J) & 14270 (J) & 3427 (J) & 5269 (J) & 12233 (J) & 14565 (J)\\
\hline
2 & 2293 (J) & 2296 (J) & 2246 (J) & 6745 (J) & 14407 (J) & 3490 (J) & 5368 (J) & 12519 (J) & 14967 (J) \\
\hline
4 & 2069 (J) & 2064 (J) & 1914 (J) & 5906 (J) & 11836 (J) & 3122 (J) & 4528 (J) & 10493 (J) & 12451 (J) \\
\hline
Average & 2202 (J) & 2189 (J) & 2119 (J) & 6406 (J) & 13504 (J) & 3346 (J) & 5055 (J) & 11748 (J) & 13995 (J) \\
\hline
\end{tabularx}
\caption{Energy consumption results for different video object detection solutions under different power modes on Jetson Xavier NX. We run all models on a randomly selected video dataset which includes 828 frames.} %For the calculation of energy, we use Eq.~\ref{eq:energy-sum}.}
\label{tab:energy}
\end{table*}
\end{comment}

\begin{table}[th!]
\centering
\small
\scalebox{0.67}{
    \begin{tabularx}{1.5\columnwidth}{|>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.67\hsize\centering\arraybackslash}X
    |>{\hsize=.57\hsize\centering\arraybackslash}X
    |>{\hsize=.53\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.6\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X|}
    \hline
    \textbf{Power Modes} & \textit{Fast Adapt} & \textit{FRCNN+} & \textit{YOLO+} & \textit{FRCNN} & \textit{YOLO} & \textit{REPP w\ YOLOv3} & \textit{MEGA} & \textit{SELSA 50} & \textit{SELSA 101}\\ 
    \hline
    \hline
    0 & 2244 & 2205 & 2196 & 6567 & 14270 & 3427 & 5269 & 12233 & 14565\\
    \hline
    2 & 2293 & 2296 & 2246 & 6745 & 14407 & 3490 & 5368 & 12519 & 14967 \\
    \hline
    4 & 2069 & 2064 & 1914 & 5906 & 11836 & 3122 & 4528 & 10493 & 12451 \\
    \hline
    Avg & 2202 & 2189 & 2119 & 6406 & 13504 & 3346 & 5055 & 11748 & 13995 \\
    \hline
    \end{tabularx}
}
\caption{Energy consumption (J) on Jetson Xavier NX.} %on a randomly selected dataset.}% with 828 frames.} %For the calculation of energy, we use Eq.~\ref{eq:energy-sum}.}
\label{tab:energy}
\end{table}

\subsection{Energy Consumption Benchmark}
\label{energy-exp}

\noindent \textbf{Experiment setup}: Embedded devices 
%SC04052021: I already have the footnote about mobile and embedded devices being synonymous so you can just write either.
need to be energy efficient as in most cases they may need to run on limited power or batteries. Thus, we measure the energy consumption of our video object detection models --- \name and baselines on our mid-tier embedded device, Xavier NX using 3 different power modes [0, 2, 4], out of 5 available power mode~\cite{jetson_guide}. Power mode 0 consumes the highest power, a total of 15W, with the highest frequency setting for each of GPU, CPU, and the DL accelerator. Power mode 4 provides the lowest power level. 
% (see Table~\ref{tab:nx-power-modes}). 
All results are reported on a randomly selected video dataset with 828 frames. %Note that the other 2 Jetson devices also support different power modes. 


%We pick the Xavier NX board, which has the middle level of computational resources among our 3 devices, for the energy consumption experiment. We run all models on a randomly selected video dataset with 828 frames under 3 different power modes [0, 2, 4], as shown in Table~\ref{tab:nx-power-modes}. 

%SC040521: It should not be "Table.~\ref{XXX}". No period after Table as you are not shortening. 

% As mentioned in Sec.~\ref{subsec:embedded}, we disabled the DVFS and fixed the working frequency at the max frequency under each mode for our overall experiments.
%SC040821: Chopped for space
% From Table~\ref{tab:nx-power-modes}, we can see that different power modes provide different key parameters for the CPU, GPU, and DL Accelerator modules. \textit{Mode 0} has a 15$W$ power budget and has the max frequencies for all modules. 
%SC04052021: what is the freq for Mode O, always put numbers
% However, it only has 2 online CPU cores, which could be undesirable for multi-threaded applications. \textit{Mode 2} also has a 15$W$ power budget, its max CPU frequency is 1400MHz. %which is not the highest. 
% However, it has 6 online CPU cores and the highest max frequency for GPU and DL Accelerator. It is not surprising to see that \textit{Mode 2} will perform better when handling multi-threaded applications. In contrast, \textit{Mode 4} has a lower power budget of 10$W$, 4 online CPU cores with max frequency at 1200MHz, its max frequencies for GPU and DL Accelerator are also the lowest. It should be able save energy but may suffer in terms of the inference latency.

Under each power mode, we first measure the idle status power using {\em tegrastats}. Mode [0, 2, 4] have idle status power of [3.25, 3.38, 3.08]$W$. Then, we run each video object detection model on a randomly selected video dataset, which has 828 frames. At the same time, we record the energy consumption by using {\em tegrastats}. The results are shown in Fig.~\ref{fig:energy} and Table.~\ref{tab:energy}. Since the major part of power consumption comes from the GPU module, and \name, FRCNN+, YOLO+ are adaptive models leveraging a lighter-weight tracker, we notice significant oscillations in their energy plots [Fig.~\ref{fig:energy}]. This is because the object tracker mainly uses the CPU and the dips in the curve happen when the tracker is executing. %Because these model do not do object detection on every frame. 
% All the green curves represent \textit{Mode 4} (power budget = 10$W$) and we can see from Fig.~\ref{eq:energy} and Table.~\ref{tab:energy} that 
We see that Mode 4 helps reduce the instantaneous power by around 33\% and total energy consumption by around 10\%. Among all models, \name, FRCNN+, and YOLO+ have the lowest average total energy consumption at around 2,200 $J$. %, this benefit from their employment of object tracker. 
REPP with YOLOv3 (baseline) consumed 3,346 $J$ on average while SELSA has the highest average energy consumption of 13,995 $J$, 6X larger than adaptive models. %For video object detection on mobile or embedded devices, we don't only need to consider the latency and accuracy, but also should consider the energy issue. Thus our benchmarking work provides insight into both adaptive models and SOTA models.
Thus, our energy benchmarking experiments validate our insight that adaptive variants of YOLO and FRCNN, as well as \name demonstrate the highest energy efficiency in comparison to their rigid counterparts. %, \eg YOLO and FRCNN and SELSA baseline.
% \pengcheng{04/05/2021 23:33 Updated， please have a pass}
%SC040521: Done
% As that cannot separate the power consumption application-wise, we exclude the use of the contention generator for the energy experiments. For the energy consumption experiment, we add another power mode by selecting the mid-point of frequency for the processor.
%SC040421: I do not understand the above sentence.
% \pengcheng{04/05/2021 04/05/2021 06:49 Rewrite the energy consumption subsection}

\begin{figure}[th!]
    \centering
    \includegraphics[width=1\linewidth]{figures/energy.png}
    \caption{Instantaneous power on Xavier NX.} 
    % We initiate the NVIDIA tegrastats module followed by the video object detection models and report the power measured every 1 second during the inference.
    % PW: Mentioned in text
    \label{fig:energy}
\end{figure}

% \jay{Add content to explain the energy consumption results.}

% \jay{Need to sync for more details on the energy experiment.
% \begin{enumerate}
%     \item include results only for one board with the full energy consumed(GPU+CPU+all components) for a fair comparison, without contention.
%     \item add 1 or 2 more power modes
%     \somali{For the power modes, add the insight as to why we are doing it}
% \end{enumerate}
% }
% \pengcheng{04/05/2021 05:12 Addressed}



==> old_files_temp/5-sec_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
\begin{comment}
\pengcheng{We have 4 dimensions to do comparison: object detection models, contention levels, devices, power modes. To compare each dimension, we need to fix other dimensions.
\begin{itemize}
    \item Different models, same board, same contention level, same max power mode
    % 100 \% power correct? \PW{04/05/2021 06:23 Yes}
    \item Different contention levels, same model, same device, same max power mode
    \item Different boards, same model, same contention level, same max power mode    
    \item 3 different power modes, same model, same device, no contention
\end{itemize}
}
\end{comment}
In this paper, we benchmark the state-of-the-art video object detection frameworks on the NVIDIA Jetson family of embedded devices under different GPU contention and power-mode scenarios. We show the latency, accuracy, and power consumption of \name compared with other video object detection models under each scenario. 
% There are 3 main variables in our benchmarking platforms: devices, GPU contention levels, and power modes. 
% Thus, our work provides insight into the performance of these models under GPU resource-constrained or power-constrained scenarios. %The GPU contention generator is a program that can occupy a certain level of GPU resources which makes it is possible to simulate real applications. 
% For different power-modes, we use the API provided by NVIDIA for the Jetson class of devices. 
According to our observation, \name provides the best Pareto frontier of accuracy-vs-latency for all three boards and under all contention levels. However, if there are loose latency bounds, among adaptive models, FRCNN+ (\ie FRCNN coupled with a tracker) achieves the highest accuracy while among non-adaptive models, SELSA outperforms all others. For the most well-resourced board, the AGX Xavier, and under the most stringent latency requirement, \name is able to sustain 76 fps in the no-contention scenario, while on Xavier NX, it is 74 fps, and on Jetson TX2, it is 38 fps. 
Among the latest video object detection models, SELSA achieves the highest mAP (81.5\%, with ResNet-101) but also suffers from a high latency ($>$ 2 seconds per frame). Also these models, SELSA, MEGA, and REPP, are not adaptive, and therefore, suffer in latency when faced with any level of contention. We also perform energy consumption experiments and find that \name, FRCNN+, and YOLO+ achieve the best, and comparable, energy efficiency, while SELSA has 6X the energy consumption of these best-in-class protocols. Thus, if one runs the boards at the lowest power level, it does not always translate to equivalent energy savings. We hope that this work points to much further work in understanding the suitability of various object detection heads on embedded boards. The understanding must encompass varying levels of resource availability on these devices as well as varying power levels of operation. 

%\pagebreak

% At the same time, it consumed the most energy when it is running video object detection workloads. 
%TX2 and Xavier NX have the same price while Xavier NX has a overall better hardware specifications and can provide lower inference latency for video object detection. 
% Finally, we found that the different power modes of Xavier NX can be leveraged to limit the working frequency of CPU, GPU, and Memory modules, in turn saving energy. %SC04052021: which power modes and how much energy does it save by switching from the highest power mode to the lowest one that we tested on a sample board (Xavier NX?), everything else remaining the same.

==> old_sec_benchmark.tex <==
\section{Benchmarking SOTA Models and Systems}
\label{sec:evaluation}


\subsection{Video Object Detection Models and Our Enhancement}

We consider 6 SOTA models for video object detection with a total of 13 protocols (including variants of the same model) for our benchmark. These models are selected using the following criteria,
\begin{enumerate}
    \item The code and model could be deployed on a Jetson TX2 board, and
    \item The model is open-sourced and the pretrained weights on the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) 2015 VID dataset~\cite{ILSVRC15} are available to reproduce the results.
%SC102021: The second reason is a weak point of our paper. A reviewer may say take the real SOTA and train on your dataset if you need to. 

\end{enumerate}

% These models can be divided into two groups.
The detailed explanation of the models are as follow.

% Jay:  Left informative comments
% For our benchmark experiments, we implement the SOTA adaptive models for video object detection along with some popular models screened using the following criteria. 1) The code and model could be deployed on an NVIDIA Jetson TX2 board, which has the lowest computation power in our device selection. We used it at the peak power level of 15W, with an AI performance of 1.33 TFLOPS. 2) The model is open-sourced and the pretrained weights on the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) 2015 VID dataset~\cite{ILSVRC15} are available.

% Jay: 10/26
% TODO: chop off 20%, 90% contention.


\noindent{\bf Adaptive video object detection models}: We implement and evaluate a total of 6 adaptive video object detection models. \name, which is our in-house variant of ApproxDet~\cite{xu2020approxdet}, sped up using our optimization in frame decoding, image resizing, and improved library APIs to represent a state-of-the-art adaptive protocol. FRCNN+ and YOLO+ in our improvement over FRCNN~\cite{ren2015faster} and YOLO~\cite{redmon2016you, redmon2018yolov3} for commonly used object detection models. In addition, SSD+ in our improvement over an SSD model, which is combined with MobileNetv2 as the feature extractor and MnasFPN~\cite{chen2020mnasfpn} for object detection, represents an efficient model variant aimed for embedded devices. 
% ApproxDet-SenSys on TX2: 80 msec ~ 300 msec latency requirement
% Fastadapt-EMDL on TX2: 33.3 msec ~ 100 msec latency requirement
% Accuracy stay the same

\noindent{\bf FRCNN+}: We added two tuning knobs for FRCNN: 1) image shape, and 2) number of proposals. Medianflow  tracker~\cite{kalal2010forward} was employed for acceleration. With different combinations of the image shape and number of proposals, there are 28 branches with the shape in the following set [224, 320, 448, 576] and number of proposals in the following set [1, 3, 5, 10, 20, 50, 100]. We used the MedianFlow tracker to speed up while keeping a sampling interval of 8 frames for the object detector. 

\noindent{\bf YOLO+}: We included one tuning knob for YOLO, which is the shape of the input image, and also used it in tandem with the MedianFlow object tracker~\cite{kalal2010forward} for acceleration. There are a total of 12 branches with the shape in the following set [224, 256, 288, 320, 352, 384, 416, 448, 480, 512, 544, 576]. Similarly, object detection was triggered every 8 frames, which is the sampling interval knob in our \name implementation and kept constant in YOLO+.

\noindent{\bf SOTA video object detection models}:
Several latest video detection models are considered to provide baseline experiments of non-adaptive models. REPP comes with a total of three model (baseline) variants - YOLOv3, SELSA, FGFA - and only their implementation of the YOLOv3 baseline was able to run on a TX2 board. We address the baseline model as YOLOv3 to avoid confusion with our own YOLO implementations (PyTorch YOLO and YOLO+), and the full model with the post-processing technique as REPP+YOLOv3. MEGA is provided with two different backbone models with different levels of features usage. Here, we use the BASE model provided by the authors with ResNet-50 as the feature extractor, as this was the only configuration that could be run on the TX2 board. We call this model MEGA base. For SELSA, we utilize ResNet-50 and ResNet-101, with the corresponding variants referred to as SELSA 50 and SELSA 101.
%
% Jay : Added efficient backbone without tuning knob.
% Jay : Pengcheng can check here and add more details later.
We also consider selected models from the SOTA object detection model EfficientDet~\cite{tan2020efficientdet}. 
\jay{There are eight models from D0 to D7, having different scaling factor that gives different depth, width, and image resolution for the network.
% \saurabh{Say how they are different.}
% Jay: 10/12/2021 : Addressed.
Our observation is that, heavier model variants above D3 cannot run on the Jetson TX2 board due to insufficient memory, thus we select lighter models D0 and D3 for the benchmark comparison.} The models are originally trained on COCO datasets and we fine-tune these models on our evaluation datasets (Sec.~\ref{sec:training_efficientdet}).
\somali{We only use D0 and D3. Mention that and argue for our choice.}
% Jay (07/08/2021) : Relocated this section(originally section 3.4), because I thought explaining the boards and power modes should come before the experiment for energy consumption part.
\somali{This description of EfficientDet is relevant for Sec 5. So I think this needs to come toward the beginning of that section.}

\subsection{Accuracy and Latency Benchmark}

\noindent \textbf{Experiment setup}: We evaluate each object detection model on our 3 embedded devices under [0, 20, 50, 90]\% GPU contention on the ILSVRC VID 2015 validation set, as is standard practice. 
%SC102021: I don't think evaluating with contention is standard practice.
% Jay 10/25: The above sentence was intended to say that evaluating on the ILSVRC val set is a standard practice.
%
For adaptive video object detection models, we consider a streaming setting for inference with video frames fed one-by-one, and report the mean latency per video frame. For other methods, we use batch processing for inference.
\somali{A reviewer may question how it is fair to compare latency or accuracy between streaming mode and batch mode.}
Fig.~\ref{fig:accuracy_latency_TX2},~\ref{fig:accuracy_latency_NX},~\ref{fig:accuracy_latency_AGX}, and~\ref{fig:sota} summarize our main results. 
%SC102021: A general rule of thumb is a figure should not come so much before it is referred. I moved the figures later. 
% In Fig.~\ref{fig:accuracy_latency_TX2}, ~\ref{fig:accuracy_latency_NX}, ~\ref{fig:accuracy_latency_AGX}, and~\ref{fig:sota} we show the latency and accuracy experiment of adaptive video object detection models on ILSVRC VID 2015 validation dataset on different devices. We run these protocols in a streaming manner with video frames fed one-by-one, and report the mean latency per video frame.

\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.4\textwidth}
        \includegraphics[width=1\columnwidth]{new_figures/accuracy_p95_latency2_g0_agx.png}
        \centerline{\small (a) No contention}
    \end{minipage}
    % \hfill
    \begin{minipage}[c]{0.4\textwidth}
        \includegraphics[width=1\columnwidth]{new_figures/accuracy_p95_latency2_g50_agx.png}
        \centerline{\small (c) 50\% GPU contention}
    \end{minipage}
    \caption{Benchmarking the object detection algorithms on the NVIDIA Jetson AGX Xavier.}
    \label{fig:accuracy_latency_AGX}
\end{figure*}
\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.4\textwidth}
        \includegraphics[width=1\columnwidth]{new_figures/accuracy_p95_latency2_g0_nx.png}
        \centerline{\small (a) No contention}
    \end{minipage}
    % \hfill
    \begin{minipage}[c]{0.4\textwidth}
        \includegraphics[width=1\columnwidth]{new_figures/accuracy_p95_latency2_g50_nx.png}
        \centerline{\small (c) 50\% GPU contention}
    \end{minipage}
    \caption{Benchmarking the object detection algorithms on the NVIDIA Jetson Xavier NX.}
    \label{fig:accuracy_latency_NX}
\end{figure*}
\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.4\textwidth}
        \includegraphics[width=1\columnwidth]{new_figures/accuracy_p95_latency2_g0_tx2.png}
        \centerline{\small (a) No contention}
    \end{minipage}
    % \hfill
    \begin{minipage}[c]{0.4\textwidth}
        \includegraphics[width=1\columnwidth]{new_figures/accuracy_p95_latency2_g50_tx2.png}
        \centerline{\small (c) 50\% GPU contention}
    \end{minipage}
    \caption{Benchmarking the object detection algorithms on the NVIDIA Jetson TX2.}
    % \somali{This figure is a little too small. Since there is no page budget, split this into 2X2 layout, for the 4 sub-figures.}
    % Jay 10/25 : Addressed, changed figure.
    \label{fig:accuracy_latency_TX2}
\end{figure*}

\subsubsection{Adaptive Video Object Detection Models}
Fig.~\ref{fig:accuracy_latency_TX2} reports the accuracy and latency of all models with varying contention levels on the NVIDIA Jetson TX2 board. In subfigure (a), we observe that \name has the lead in the accuracy-latency frontier over FRCNN+, YOLO+ and SSD+ over a wide range of latency budgets, varying from 33.3 msec to 200 msec. For \name, the accuracy goes up to 49.8\% mAP, running at 142.7 msec per frame (roughly 7.0 fps) and the accuracy drops by 5.6\%, running at 37.9 fps. For FRCNN+, it is able to achieve a similar accuracy to \name but the accuracy drops significantly (>15\%) as we dial up the speed to 20 fps. 
%
This is because FastAdapt provides 3 more tuning knobs than FRCNN+, and a well-designed scheduler to determine which branch to run. For YOLO+, though with lower accuracy given high latency budget (100 to 200 msec), it wins at accuracy over FRCNN+ when the latency budget is less than 100 mesec, the accuracy drop is 8\% from 150 msec speed to 50 msec speed. 
%
Lastly for SSD+, the accuracy is at maximum of 48.6\% with a latency of 124.4 msec per frame. Due to its efficient backbone, 
%SC102021: English issue should be "its efficient backbone"
the fully featured model already has a low latency. The latency varies from 50.2 msec to 124.4 msec per frame, and accuracy drops down to 35.9\% with the fastest latency configuration. These observations with efficient adaptive models show the ability of \name to provide a much better trade-off in accuracy vs. latency.
%
Finally, we also show that latency and accuracy of FRCNN and YOLO without our optimization in the figure, where the latency axis is in log-scale. For FRCNN and YOLO, the latency is 693 and 1051 msec per frame while the accuracy is 51.1\% and 49.5\%, respectively. For SSD, the latency is 124.4 msec per frame while the accuracy is 48.6\%. Even if the SSD model uses an input image size of 320 by default, the latency value is superior compared with FRCNN or YOLO while maintaining a relatively high accuracy.

In subfigures (b), (c), (d), we measure the performance of these protocols under GPU contention. Compared to subfigure (a), we observe that \name maintains the latency with reduced accuracy and superior to FRCNN+, YOLO+, and SSD+ validating its claim of approximation at runtime to resource availability. Given a 50\% GPU contention, \name's accuracy drop is 7.8\% given a 30 fps speed and 1.0\% given a 5 fps speed. In contrast, FRCNN+, YOLO+ and SSD+ are 1.4X-2X slower with 50\% to 90\% GPU contention.
%SC102021: To provide an apples-to-apples comparison, you should report on accuracy drop for the baselines. 

On Xavier NX and AGX Xavier devices, we set the latency budget as [20, 33, 50, 100, 200] msec for Xavier NX and [20, 33, 50, 100] msec for AGX Xavier based on their higher computational capabilities than Jetson (also, recall that AGX Xavier $>$ Xavier NX). In most cases \name is superior at both accuracy and latency to FRCNN+, YOLO+, and SSD+. As we can see the results on Xavier NX from Fig.~\ref{fig:accuracy_latency_NX}, in subfigure (a), \name achieves 49.3\% accuracy with 59.3 msec per frame (16.9 fps), and accuracy drops to 43.9\% running at 28.4 msec per frame (35.2 fps). FRCNN+ is comparable to or even better than \name when the latency budget is sufficient. However, the accuracy drops quickly to 40.9\% when it speeds up to 27.8 msec (36.0 fps). YOLO+ has an accuracy of 44.2\% when  running at 52.2 msec per frame (19.2 fps), and SSD+ has an accuracy of 31.9\% when the latency is 36.7 msec  (27.2 fps).
%
We further add GPU contention for the latency-accuracy experiment, in subfigure (b), (c), (d), the overall latency of \name, FRCNN+, YOLO+, and SSD+ increase as the contention increase from 0\% to 90\%. However, \name can still keep the fps at 16 fps with accuracy of 46\% when there is 50\% GPU contention. 
%
With the increased hardware computational capability, Fig.~\ref{fig:accuracy_latency_AGX} shows that all models achieve roughly 2 times higher fps on AGX Xavier compared to that on TX2. \name can achieve 47.5\%  accuracy when running at 20.1 msec per frame (49.8 fps). On the other hand, FRCNN+ can achieve 41.9\% accuracy when running at 20.2 msec per frame (49.5 fps) and YOLO+ can achieve 39.9\% when running at 23.3 msec per frame (42.9 fps). SSD+ is able to show better trade-off on a more powerful board, and can achieve 31.9\% at 35.9 fps.
%
% Jay (07/09/2021) Moved this line to the end to emphasize FastAdapt's performance.
Overall, even when compared with efficient models, \name leads the accuracy performance when the latency budget is limited (from 20 msec to 50 msec)

% Jay: Add content for explaining more on the observations.
% Jay (07/06/2021) Write up for Additional Observations.
To summarize, all 3 groups of experiments suggest that as contention increased, the accuracy is influenced and will drop accordingly. \name leads the latency-accuracy in all scenarios especially under stringent latency requirements. Compared to tunable model variants (FRCNN+, YOLO+, and SSD+), \name is able to schedule the tuning knob with more options, especially with the sampling interval that controls how often the object tracker is triggered. The object tracker uses much less GPU resources, compared to the object detector, and suffers relatively lower accuracy loss for most cases where the tracking of the objects are not lost. This gives \name the ability to meet the latency requirement more flexibly while maintaining higher accuracy than other tunable model variants. We also observe that the latency of SSD+ models are not impacted by contention when the resource usage is small, e.g., using a tracker and small image shape, or the board is powerful enough to run the model along the contention. The likely explanation is that the GPU resources consumed by the SSD+ model is small enough not to get impacted by the contention.

\begin{figure*}[t]
    \centering
    \begin{minipage}[c]{0.32\textwidth}
        \includegraphics[width=1\columnwidth]{figures/tx2_contention_performance.png}
        \centerline{\small (a) Jetson TX2}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.32\textwidth}
        \includegraphics[width=1\columnwidth]{figures/nx_contention_performance.png}
        \centerline{\small (b) Jetson Xavier NX}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.32\textwidth}
        \includegraphics[width=1\columnwidth]{figures/agx_contention_performance.png}
        \centerline{\small (c) Jetson AGX Xavier}
    \end{minipage}
    \caption{Benchmarking SOTA video object detection models on NVIDIA Jetson Devices under different contention levels. The accuracy measurements are the same among all boards and are as follows. EfficientDet D0: 48.62\% mAP, EfficientDet D3: 58.32\% mAP, YOLOv3: 51.25\% mAP, REPP+YOLOv3: 74.81\% mAP, MEGA base: 68.11\% mAP, SELSA 50: 77.31\% mAP, SELSA 101: 81.5\% mAP.}
    \label{fig:sota}
\end{figure*}

\subsubsection{Video Object Detection Models}
Both SOTA models (YOLOv3, REPP+YOLOv3, MEGA base, SELSA 50, 101) and efficient models (EfficientDet-D0, EfficientDet-D3) are experimented for accuracy and latency on different embedded devices. As we can see from the caption of Fig.~\ref{fig:sota}, without latency budgets, SOTA models achieve higher mAP than most adaptive models, ranging from 51.3\% to 81.5\%, while on the other hand, EfficientDet-D0 and EfficientDet-D3 achieves 48.6\% and 58.3\% respectively. For latency results, EfficientDet-D0 has the lowest latency among all models, and YOLO has the lowest mAP on all boards in line with prior works. SELSA 101 achieves the highest mAP but with the highest latency on all boards. In contrast, REPP+YOLOv3 has a superior mAP at 74.81\% while still maintaining a low latency. EfficientDet-D3 runs at a similar speed of MEGA, but has a much lower accuracy.
% Ran (06/08/2021): weakness of our EfficientDet models, commented
% As we have trained the EfficientDet models ourselves without rigorous exploration to push the accuracy higher, there may be more space for EfficientDet models to perform better. The last point is that on all devices, these SOTA models follow a similar trend of increased accuracy with higher latency.
The accuracy values obtained in our benchmark for SOTA models differ from those of the original authors, most significantly for REPP. This we believe is due to two reasons---first, we use an IoU threshold of 0.6 consistently for all protocols (original authors use different thresholds for different protocols---0.5 for REPP) and second, for the REPP evaluation, we use the code's ``demo" version, rather than the ``full" version, which has most parameter values hard-coded and thus not easy to use. 
%
We find from our evaluation that the SOTA models all suffer from poor latency, further exacerbated under GPU contention, showing up to 2X increased latency with contention over 50\%. This is because of their model sizes and inability to adapt to contention. 
%
In addition, the EfficientDet-D0 model could achieve a latency of 103.3 msec on the TX2 board. However, unlike SSD+ which is a similarly light model, it is still impacted more than twice under contention, implying the effectiveness of \name's implementation of tuning knobs for adaptive models.

\begin{comment}
\begin{table*}[ht!]
\centering
\small
\begin{tabularx}{\textwidth}{|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X
|>{\hsize=.4\hsize\centering\arraybackslash}X|}
\hline
\textbf{Power Modes ID} & \textbf{FastAdapt} & \textbf{FRCNN+} & \textbf{YOLO+} & \textbf{FRCNN} & \textbf{YOLO} & \textbf{REPP w\ YOLOv3} & \textbf{MEGA} & \textbf{SELSA 50} & \textbf{SELSA 101}\\ 
\hline
\hline
0 & 2244 (J) & 2205 (J) & 2196 (J) & 6567 (J) & 14270 (J) & 3427 (J) & 5269 (J) & 12233 (J) & 14565 (J)\\
\hline
2 & 2293 (J) & 2296 (J) & 2246 (J) & 6745 (J) & 14407 (J) & 3490 (J) & 5368 (J) & 12519 (J) & 14967 (J) \\
\hline
4 & 2069 (J) & 2064 (J) & 1914 (J) & 5906 (J) & 11836 (J) & 3122 (J) & 4528 (J) & 10493 (J) & 12451 (J) \\
\hline
Average & 2202 (J) & 2189 (J) & 2119 (J) & 6406 (J) & 13504 (J) & 3346 (J) & 5055 (J) & 11748 (J) & 13995 (J) \\
\hline
\end{tabularx}\vspace{-0.5em}
\caption{Energy consumption results for different video object detection solutions under different power modes on Jetson Xavier NX. We run all models on a randomly selected video dataset which includes 828 frames.}
\label{tab:energy}
\end{table*}

\begin{table}[th!]
\centering
\small
\scalebox{0.67}{
    \begin{tabularx}{1.5\columnwidth}{|>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.40\hsize\centering\arraybackslash}X
    |>{\hsize=.40\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.67\hsize\centering\arraybackslash}X
    |>{\hsize=.57\hsize\centering\arraybackslash}X
    |>{\hsize=.53\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.6\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X|}
    \hline
    \textbf{Power Modes} & \textit{Fast Adapt} & \textit{FRCNN+} & \textit{YOLO+} & \textit{SSD} & \textit{SSD+} & \textit{EffDet D0} & \textit{EffDet D3} & \textit{FRCNN} &\textit{YOLO} & \textit{REPP w\ YOLOv3} & \textit{MEGA} & \textit{SELSA 50} & \textit{SELSA 101}\\ 
    \hline
    \hline
    0 & 2244 & 2205 & 2196 & 692 & 295 & 1050 & 4786 & 6567 & 14270 & 3427 & 5269 & 12233 & 14565\\
    \hline
    2 & 2293 & 2296 & 2246 & 757 & 346 & 1183 & 5050 & 6745 & 14407 & 3490 & 5368 & 12519 & 14967 \\
    \hline
    4 & 2069 & 2064 & 1914 & 716 & 347 & 1025 & 4323 & 5906 & 11836 & 3122 & 4528 & 10493 & 12451 \\
    \hline
    Avg & 2202 & 2189 & 2119& 722 & 329 & 1086 & 4720 & 6406 & 13504 & 3346 & 5055 & 11748 & 13995 \\
    \hline
    \end{tabularx}
}
\caption{Energy consumption (J) on Jetson Xavier NX.}
\label{tab:energy}
\end{table}
\end{comment}

\begin{table}[th!]
\centering
\small
\scalebox{0.67}{
    \begin{tabularx}{1.5\columnwidth}{|>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.62\hsize\centering\arraybackslash}X
    |>{\hsize=.40\hsize\centering\arraybackslash}X
    |>{\hsize=.40\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.6\hsize\centering\arraybackslash}X
    |>{\hsize=.62\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.53\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X
    |>{\hsize=.45\hsize\centering\arraybackslash}X|}
    \hline
    \textbf{Power Modes} & \textit{SSD+} & \textit{SSD} & \textit{EffDet D0} & \textit{YOLO+} & \textit{FRCNN+} & \textit{Fast Adapt} & \textit{REPP w\ YOLOv3} &   \textit{EffDet D3} & \textit{MEGA} & \textit{FRCNN} & \textit{SELSA 50} &\textit{YOLO} & \textit{SELSA 101}\\ 
    \hline
    \hline
    0 & 295 & 692 & 1050 & 2196 & 2205 & 2244 & 3427 & 4786 & 5269 & 6567 & 12233 & 14270 & 14565\\
    \hline
    2 & 346 & 757 & 1183 & 2246 & 2296 & 2293 & 3490 & 5050 & 5368 & 6745 & 12519 & 14407 & 14967 \\
    \hline
    4 & 347 & 716 & 1025 & 1914 & 2064 & 2069 & 3122 & 4323 & 4528 & 5906 & 10493 & 11836 & 12451 \\
    \hline
    Avg & 329 & 722 & 1086 & 2119& 2189 & 2202 & 3346 & 4720 & 5055 & 6406 & 11748 & 13504 & 13995 \\
    \hline
    \end{tabularx}
}
\caption{Energy consumption (J) on Jetson Xavier NX.}
\label{tab:energy}
\end{table}

\subsection{Energy Consumption Benchmark}\label{energy-exp}

For the energy consumption experiments, we explicitly choose the Jetson NX board as it is a middle class device among our device selection with a moderate level of power modes. From the total of five power modes shown in Table~\ref{tab:nx-power-modes}, we select power mode 0, 2, and 4 in our experiments to cover most usage scenarios, and observe the impact of different power budget and processor configurations on energy consumption.

\begin{figure}[th!]
    \centering
    \includegraphics[width=1\linewidth]{figures/energy.png}
    \caption{Instantaneous power on Xavier NX.} 
    \label{fig:energy}
\end{figure}


\noindent \textbf{Experiment setup}: Embedded devices 
need to be energy efficient as in most cases they may need to run on limited power or batteries. Thus, we measure the energy consumption of our video object detection models---\name and baselines on our mid-tier embedded device, Xavier NX using 3 different power modes [0, 2, 4], out of 5 available ones~\cite{jetson_guide}. 
\begin{table}[ht!]
    \centering
    \small
    \begin{tabularx}{\columnwidth}{|>{\hsize=0.4\hsize\centering\arraybackslash}X
    |>{\hsize=.1\hsize\centering\arraybackslash}X
    |>{\hsize=.1\hsize\centering\arraybackslash}X
    |>{\hsize=.1\hsize\centering\arraybackslash}X
    |>{\hsize=.1\hsize\centering\arraybackslash}X
    |>{\hsize=.1\hsize\centering\arraybackslash}X|}
        \hline
        \textbf{Key Parameters} & \textbf{Power Mode 0} & \textbf{Power Mode 1} & \textbf{Power Mode 2} & \textbf{Power Mode 3} & \textbf{Power Mode 4}\\ 
        \hline
        \hline
        Power Budget & 15W & 15W & 15W & 10W & 10W \\
        \hline
        Online CPU Cores & 2 & 4 & 6 & 2 & 4 \\
        \hline
        Maximal CPU Frequency (MHz) & 1900 & 1400 & 1400 & 1500 & 1200 \\
        \hline
        Maximal GPU Frequency (MHz) & 1100 & 1100 & 1100 & 800 & 800 \\
        \hline
        %DL Accelerator cores & 2 & 2 & 2 & 2 & 2 \\
        %\hline
        Maximal DL Accelerator Frequency (MHz) & 1100 & 1100 & 1100 & 900 & 900 \\
        \hline
        %Maximal Memory Frequency (MHz) & 1600 & 1600 & 1600 & 1600 & 1600 \\
        %\hline
    \end{tabularx}
    \caption{Different Power Modes for Jetson Xavier NX.}\label{tab:nx-power-modes}
\end{table}
% \somali{This table can be removed since we do not give energy experiments on the Xavier NX.}
% Ran (10/20/2021): we do have. So keep it.

% Power mode 0 consumes the highest power (15W), with the highest frequency setting for each of GPU, CPU, and the DL accelerator. Power mode 4 provides the lowest power level. 
As can be seen from Table~\ref{tab:nx-power-modes}: power mode 0 provides the highest power budget (15W), with the highest frequency setting for each of GPU, CPU, and the deep learning accelerator; power mode 2 also provides a 15W power budget, with the CPU frequency setting lower than mode 0, and having 6 CPU cores enabled compared to only 2 CPU cores in mode 0. Power mode 4 provides the lowest power budget (10W) and lowest frequency setting for each module.

% Jay : Kept informative comments.
% Note that the other 2 Jetson devices also support different power modes. 
%We pick the Xavier NX board, which has the middle level of computational resources among our 3 devices, for the energy consumption experiment. We run all models on a randomly selected video dataset with 828 frames under 3 different power modes [0, 2, 4], as shown in Table~\ref{tab:nx-power-modes}. 
% However, it only has 2 online CPU cores, which could be undesirable for multi-threaded applications. \textit{Mode 2} also has a 15$W$ power budget, its max CPU frequency is 1400MHz. %which is not the highest. 
% However, it has 6 online CPU cores and the highest max frequency for GPU and DL Accelerator. It is not surprising to see that \textit{Mode 2} will perform better when handling multi-threaded applications. In contrast, \textit{Mode 4} has a lower power budget of 10$W$, 4 online CPU cores with max frequency at 1200MHz, its max frequencies for GPU and DL Accelerator are also the lowest. It should be able save energy but may suffer in terms of the inference latency.

Under each power mode, we first measure the idle status power using {\em tegrastats}. Mode [0, 2, 4] have idle status power of [3.25, 3.38, 3.08]$W$. Then, we run each video object detection model on a randomly selected video dataset, which has 828 frames. At the same time, we record the energy consumption using {\em tegrastats}. The results are shown in Fig.~\ref{fig:energy} and Table~\ref{tab:energy}.

\subsubsection{Energy Consumption of Different Video Object Detection Models}

Since the major part of power consumption comes from the GPU module, and \name, FRCNN+, YOLO+ leverage an object tracker in our adaptive versions, we notice significant oscillations in their energy plots (Fig.~\ref{fig:energy}). This is because the object tracker mainly uses the CPU which is more energy efficient. The switching between object detector (mainly executed on GPU) and object tracker (mainly executed on GPU) corresponds to the oscillations in the curve. On the other hand, while SSD+ is also leveraging an object tracker with the detector, does not show as many oscillations as \name, FRCNN+, and YOLO+. The reason is that the default image shape knob we use for SSD+ is much smaller---320 at max, compared to 576 for \name, FRCNN+ and YOLO+ resulting in a smaller change between using detector and tracker. Also the model's efficient design with fewer numbers of parameters contributes to smaller energy consumption using the GPU, making the difference of using a tracker marginal.

% Ran (10/21/2021): check again the results of this section and how we present considering Sec. 5.
\jay{Efficient models (SSD, SSD+, EfficientDet-D0) consume lower instantaneous power as measured in real-time. As shown in Figure~\ref{fig:energy}, The maximum peak power and the overall power level during inference is much lower up to 33\%, compared to other models.}

% All the green curves represent \textit{Mode 4} (power budget = 10$W$) and we can see from Fig.~\ref{eq:energy} and Table~\ref{tab:energy} that 


Among all models, SSD, SSD+ and EfficientDet-D0 has a superior performance energy-wise, especially with SSD+ having less than 350 $J$, proving that using an efficient backbone reduces energy consumption by a large ratio. In addition, \name, FRCNN+, and YOLO+ have low average total energy consumption compared to SOTA models at around 2,200 $J$. REPP with YOLOv3 (baseline) consumed 3,346 $J$ on average while SELSA has the highest average energy consumption of 13,995 $J$, 6X larger than adaptive models. Our overall energy benchmarking experiments validate our insight that adaptive models FRCNN+, YOLO+, and SSD+, as well as \name demonstrate better energy efficiency relative to their rigid variants. 

%For video object detection on mobile or embedded devices, we don't only need to consider the latency and accuracy, but also should consider the energy issue. Thus our benchmarking work provides insight into both adaptive models and SOTA models.

\subsubsection{Energy Consumption of Different Power Modes}

Total of three different power modes - 0, 2, 4 - from the NX board were selected to further explore the impact of different board configurations on the energy consumption.
%Power mode-wise, 
We can see from Fig.~\ref{fig:energy} and Table~\ref{tab:energy} that all models in power mode 0 achieve lower latency than that in power mode 2 and 4, with the overall highest energy consumption. This is because of its higher hardware frequency settings. All models in power mode 4 has the slowest inference latency with the lowest instantaneous power level compared with that in power mode 0 and 2. Particularly, compared with mode 0, power mode 4 helps reduce the instantaneous power on average over models, by around 30\% and total energy consumption by around 10\% despite it's longer average inference time of 18\%.
Our observation on the energy consumption difference between different power modes suggests that the power mode could be adjusted according to the user requirements. Specifically, for video object detection tasks, 
the users can make their choice whether to focus on latency performance by choosing a higher performance power mode (\eg mode 0) or energy saving by switching to a lower performance power mode (\eg mode 4) of the embedded devices.

% \begin{figure}[th!]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/energy.png}
%     \caption{Instantaneous power on Xavier NX.} 
%     % We initiate the NVIDIA tegrastats module followed by the video object detection models and report the power measured every 1 second during the inference.
%     % PW: Mentioned in text
%     \label{fig:energy}
% \end{figure}

